Formation and desorption of sulfur chains (H$_2$S$_x$ and S$_x$) in cometary ice: effects of ice composition and temperature

The reservoir of sulfur accounting for sulfur depletion in the gas of dense clouds and circumstellar regions is still unclear. One possibility is the formation of sulfur chains, which would be difficult to detect by spectroscopic techniques. This work explores the formation of sulfur chains experimentally, both in pure H$_2$S ice samples and in H$_2$O:H$_2$S ice mixtures. An ultra-high vacuum chamber, ISAC, eqquipped with FTIR and QMS, was used for the experiments. Our results show that the formation of H$_2$S$_x$ species is efficient, not only in pure H$_2$S ice samples, but also in water-rich ice samples. Large sulfur chains are formed more efficiently at low temperatures ($\approx$10 K), while high temperatures ($\approx$50 K) favour the formation of short sulfur chains. Mass spectra of H$_2$S$_x$, x~=~2-6, species are presented for the first time. Their analysis suggests that H$_2$S$_x$ species are favoured in comparison with S$_x$ chains. Nevertheless, the detection of several S$_x^+$ fragments at high temperatures in H$_2$S:H$_2$O ice mixtures suggests the presence of S$_8$ in the irradiated ice samples, which could sublimate from 260~K. ROSINA instrument data from the cometary Rosetta mission detected mass-to-charge ratios 96 and 128. Comparing these detections with our experiments, we propose two alternatives: 1) H$_2$S$_4$ and H$_2$S$_5$ to be responsible of those S$_3^+$ and S$_4^+$ cations, respectively, or 2) S$_8$ species, sublimating and being fragmented in the mass spectrometer. If S$_8$ is the parent molecule, then S$_5^+$ and S$_6^+$ cations could be also detected in future missions by broadening the mass spectrometer range.

==> bibliography.tex <==
%UTILIZADOS PARA EL PAPER DEL CO Y CO2 MEZCLADOS CON N2
%
%
%
%
%
%
%

@ARTICLE{Gerakines1996,
       author = {{Gerakines}, P.~A. and {Schutte}, W.~A. and {Ehrenfreund}, P.},
        title = "{Ultraviolet processing of interstellar ice analogs. I. Pure ices.}",
      journal = {\aap},
     keywords = {ISM: MOLECULES, DUST, EXTINCTION, INFRARED: ISM: LINES AND BANDS,
        MOLECULAR DATA, MOLECULAR PROCESSES, METHODS: LABORATORY},
         year = 1996,
        month = Aug,
       volume = {312},
        pages = {289-305},
       adsurl = {https://ui.adsabs.harvard.edu/#abs/1996A&A...312..289G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

      
@ARTICLE{MD2015,
       author = {{Mart{\'\i}n-Dom{\'e}nech}, R. and {Manzano-Santamar{\'\i}a}, J. and
        {Mu{\~n}oz Caro}, G.~M. and {Cruz-D{\'\i}az}, G.~A. and {Chen},
        Y. -J. and {Herrero}, V.~J. and {Tanarro}, I.},
        title = "{UV photoprocessing of CO$_{2}$ ice: a complete quantification of
        photochemistry and photon-induced desorption processes}",
      journal = {\aap},
     keywords = {ISM: molecules, ISM: clouds, methods: laboratory: solid state,
        techniques: spectroscopic, Astrophysics - Solar and Stellar
        Astrophysics},
         year = 2015,
        month = Dec,
       volume = {584},
          eid = {A14},
        pages = {A14},
          doi = {10.1051/0004-6361/201526003},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/#abs/2015A&A...584A..14M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Smith2018,
   author = {{Smith}, L.~R. and {Panto}, E.~M. and {Gudipati}, M.~S. and 
	{Smith}, R.~L.},
    title = "{Exploring 12CO/13CO Ice-Gas Fractionation Through Interstellar Ice-Analog Experiments}",
booktitle = {Lunar and Planetary Science Conference},
     year = 2018,
   series = {Lunar and Planetary Inst.~Technical Report},
   volume = 49,
    month = mar,
      eid = {1187},
    pages = {1187},
   adsurl = {http://adsabs.harvard.edu/abs/2018LPI....49.1187S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{MD2016,
       author = {{Mart{\'\i}n-Dom{\'e}nech}, R. and {Mu{\~n}oz Caro}, G.~M. and
        {Cruz-D{\'\i}az}, G.~A.},
        title = "{Study of the photon-induced formation and subsequent desorption of
        CH$_{3}$OH and H$_{2}$CO in interstellar ice analogs}",
      journal = {\aap},
     keywords = {ISM: molecules, ISM: clouds, methods: laboratory: molecular,
        Astrophysics - Astrophysics of Galaxies, Astrophysics - Solar
        and Stellar Astrophysics},
         year = 2016,
        month = May,
       volume = {589},
          eid = {A107},
        pages = {A107},
          doi = {10.1051/0004-6361/201528025},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/#abs/2016A&A...589A.107M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@article{Asper2014,
  author={Y.-J. Chen and K.-J. Chuang and G. M. Muñoz-Caro and M. Nuevo and C.-C. Chu and T.-S. Yih and W.-H. Ip and C.-Y. R. Wu},
  title={Vacuum Ultraviolet Emission Spectrum Measurement of a Microwave-discharge Hydrogen-flow Lamp in Several Configurations: Application to Photodesorption of CO Ice},
  journal={The Astrophysical Journal},
  volume={781},
  number={1},
  pages={15},
  url={http://stacks.iop.org/0004-637X/781/i=1/a=15},
  year={2014},
  }

	
@article{Bertin2013,
  author={Mathieu Bertin and Edith C. Fayolle and Claire Romanzin and Hugo A. M. Poderoso and Xavier Michaut and Laurent
Philippe and Pascal Jeseck and Karin I. Öberg and Harold Linnartz and Jean-Hugues Fillion},
  title={Indirect Ultraviolet Photodesorption from CO:N2 Binary Ices — an Efficient Grain-gas Process},
  journal={The Astrophysical Journal},
  volume={779},
  number={2},
  pages={120},
  url={http://stacks.iop.org/0004-637X/779/i=2/a=120},
  year={2013},
  abstract={Ultraviolet (UV) ice photodesorption is an important non-thermal desorption pathway in many interstellar environments that has been invoked to explain observations of cold molecules in disks, clouds, and cloud cores. Systematic laboratory studies of the photodesorption rates, between 7 and 14 eV, from CO:N 2 binary ices, have been performed at the DESIRS vacuum UV beamline of the synchrotron facility SOLEIL. The photodesorption spectral analysis demonstrates that the photodesorption process is indirect, i.e., the desorption is induced by a photon absorption in sub-surface molecular layers, while only surface molecules are actually desorbing. The photodesorption spectra of CO and N 2 in binary ices therefore depend on the absorption spectra of the dominant species in the sub-surface ice layer, which implies that the photodesorption efficiency and energy dependence are dramatically different for mixed and layered ices compared with pure ices. In particular, a thin (1-2 ML) N 2 ice layer on top of CO will effectively quench CO photodesorption, while enhancing N 2 photodesorption by a factor of a few (compared with the pure ices) when the ice is exposed to a typical dark cloud UV field, which may help to explain the different distributions of CO and N 2 H + in molecular cloud cores. This indirect photodesorption mechanism may also explain observations of small amounts of complex organics in cold interstellar environments.}
}
	
@ARTICLE{Asper2007,
   author = {{Chen}, Y.-J. and {Nuevo}, M. and {Hsieh}, J.-M. and {Yih}, T.-S. and 
	{Sun}, W.-H. and {Ip}, W.-H. and {Fung}, H.-S. and {Chiang}, S.-Y. and 
	{Lee}, Y.-Y. and {Chen}, J.-M. and {Wu}, C.-Y.~R.},
    title = "{Carbamic acid produced by the UV/EUV irradiation of interstellar ice analogs}",
  journal = {\aap},
 keywords = {astrochemistry, molecular processes, methods: laboratory, techniques: spectroscopic, ISM: molecules, ultraviolet: ISM},
     year = 2007,
    month = mar,
   volume = 464,
    pages = {253-257},
      doi = {10.1051/0004-6361:20066631},
   adsurl = {http://adsabs.harvard.edu/abs/2007A%26A...464..253C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bertin2012,
       author = {{Bertin}, Mathieu and {Fayolle}, Edith C. and {Romanzin}, Claire and
        {{\"O}berg}, Karin I. and {Michaut}, Xavier and {Moudens},
        Audrey and {Philippe}, Laurent and {Jeseck}, Pascal and
        {Linnartz}, Harold and {Fillion}, Jean-Hugues},
        title = "{UV photodesorption of interstellar CO ice analogues: from subsurface
        excitation to surface desorption}",
      journal = {Physical Chemistry Chemical Physics (Incorporating Faraday Transactions)},
         year = 2012,
        month = Jan,
       volume = {14},
        pages = {9929},
          doi = {10.1039/C2CP41177F},
       adsurl = {https://ui.adsabs.harvard.edu/#abs/2012PCCP...14.9929B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Gerakines1995,
   author = {{Gerakines}, P.~A. and {Schutte}, W.~A. and {Greenberg}, J.~M. and 
	{van Dishoeck}, E.~F.},
    title = "{The infrared band strengths of H\_2\_O, CO and CO\_2\_ in laboratory simulations of astrophysical ice mixtures.}",
  journal = {\aap},
   eprint = {astro-ph/9409076},
 keywords = {INFRARED: ISM: LINES AND BANDS, ISM: ABUNDANCES, DUST, ISM: MOLECULES, MOLECULAR DATA, METHODS: LABORATORY},
     year = 1995,
    month = apr,
   volume = 296,
    pages = {810},
   adsurl = {http://adsabs.harvard.edu/abs/1995A%26A...296..810G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Mumma2011,
       author = {{Mumma}, Michael J. and {Charnley}, Steven B.},
        title = "{The Chemical Composition of Comets{\textemdash}Emerging Taxonomies and
        Natal Heritage}",
      journal = {Annual Review of Astronomy and Astrophysics},
         year = 2011,
        month = Sep,
       volume = {49},
        pages = {471-524},
          doi = {10.1146/annurev-astro-081309-130811},
       adsurl = {https://ui.adsabs.harvard.edu/#abs/2011ARA&A..49..471M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Prasad1983,
   author = {{Prasad}, S.~S. and {Tarafdar}, S.~P.},
    title = "{UV radiation field inside dense clouds - Its possible existence and chemical implications}",
  journal = {\apj},
 keywords = {Hydrogen Clouds, Interstellar Matter, Molecular Clouds, Radiative Transfer, Ultraviolet Radiation, Carbon Monoxide, Cosmic Rays, Interstellar Chemistry, Molecular Excitation, Photodissociation},
     year = 1983,
    month = apr,
   volume = 267,
    pages = {603-609},
      doi = {10.1086/160896},
   adsurl = {http://adsabs.harvard.edu/abs/1983ApJ...267..603P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Cecchi1992,
       author = {{Cecchi-Pestellini}, Cesare and {Aiello}, Santi},
        title = "{Cosmic ray induced photons in dense interstellar clouds}",
      journal = {\mnras},
     keywords = {Cosmic Rays, Interstellar Gas, Molecular Clouds, Particle Collisions,
        Photons, Ultraviolet Radiation, Cosmic Dust, Energy Dissipation,
        Interstellar Extinction, Astrophysics},
         year = 1992,
        month = Sep,
       volume = {258},
        pages = {125-133},
          doi = {10.1093/mnras/258.1.125},
       adsurl = {https://ui.adsabs.harvard.edu/#abs/1992MNRAS.258..125C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Oberg2007,
       author = {{{\"O}berg}, Karin I. and {Fuchs}, Guido W. and {Awad}, Zainab and
        {Fraser}, Helen J. and {Schlemmer}, Stephan and {van Dishoeck},
        Ewine F. and {Linnartz}, Harold},
        title = "{Photodesorption of CO Ice}",
      journal = {\apj},
     keywords = {Astrochemistry, ISM: Abundances, ISM: Molecules, Molecular Data,
        Molecular Processes},
         year = 2007,
        month = Jun,
       volume = {662},
        pages = {L23-L26},
          doi = {10.1086/519281},
       adsurl = {https://ui.adsabs.harvard.edu/#abs/2007ApJ...662L..23O},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Guille2010,
       author = {{Mu{\~n}oz Caro}, G.~M. and {Jim{\'e}nez-Escobar}, A. and
        {Mart{\'\i}n-Gago}, J. {\'A}. and {Rogero}, C. and {Atienza}, C.
        and {Puertas}, S. and {Sobrado}, J.~M. and {Torres-Redondo}, J.},
        title = "{New results on thermal and photodesorption of CO ice using the novel
        InterStellar Astrochemistry Chamber (ISAC)}",
      journal = {\aap},
     keywords = {ISM: clouds, ISM: molecules, molecular processes, methods: laboratory,
        infrared: ISM, techniques: spectroscopic},
         year = 2010,
        month = Nov,
       volume = {522},
          eid = {A108},
        pages = {A108},
          doi = {10.1051/0004-6361/200912462},
       adsurl = {https://ui.adsabs.harvard.edu/#abs/2010A&A...522A.108M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@BOOK{Okabe1978,
       author = {{Okabe}, Hideo},
        title = "{Photochemistry of small molecules}",
    booktitle = {A Wiley-Interscience Publication, New York: Wiley, 1978},
         year = 1978,
       adsurl = {https://ui.adsabs.harvard.edu/#abs/1978psm..book.....O},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Cottin2003,
       author = {{Cottin}, Herv{\'e} and {Moore}, Marla H. and {B{\'e}nilan}, Yves},
        title = "{Photodestruction of Relevant Interstellar Molecules in Ice Mixtures}",
      journal = {\apj},
     keywords = {Astrochemistry, ISM: Molecules, Methods: Laboratory, Molecular
        Processes, Ultraviolet: ISM},
         year = 2003,
        month = Jun,
       volume = {590},
        pages = {874-881},
          doi = {10.1086/375149},
       adsurl = {https://ui.adsabs.harvard.edu/#abs/2003ApJ...590..874C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Asper2017,
       author = {{Chen}, Y. -J. and {Mu{\~n}oz Caro}, G.~M. and {Aparicio}, S. and
        {Jim{\'e}nez-Escobar}, A. and {Lasne}, J. and {Rosu-Finsen}, A.
        and {McCoustra}, M.~R.~S. and {Cassidy}, A.~M. and {Field}, D.},
        title = "{Wannier-Mott Excitons in Nanoscale Molecular Ices}",
      journal = {\prl},
         year = 2017,
        month = Oct,
       volume = {119},
          eid = {157703},
        pages = {157703},
          doi = {10.1103/PhysRevLett.119.157703},
       adsurl = {https://ui.adsabs.harvard.edu/#abs/2017PhRvL.119o7703C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Oberg2009,
       author = {{{\"O}berg}, K.~I. and {van Dishoeck}, E.~F. and {Linnartz}, H.},
        title = "{Photodesorption of ices I: CO, N$_{2}$, and CO$_{2}$}",
      journal = {\aap},
     keywords = {astrochemistry, molecular processes, methods: laboratory, ultraviolet:
        ISM, ISM: molecules, circumstellar matter, Astrophysics},
         year = 2009,
        month = Mar,
       volume = {496},
        pages = {281-293},
          doi = {10.1051/0004-6361/200810207},
archivePrefix = {arXiv},
       eprint = {0809.1333},
 primaryClass = {Astrophysics},
       adsurl = {https://ui.adsabs.harvard.edu/#abs/2009A&A...496..281O},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Jamieson2006,
       author = {{Jamieson}, Corey S. and {Mebel}, Alexander M. and {Kaiser}, Ralf I.},
        title = "{Understanding the Kinetics and Dynamics of Radiation-induced Reaction
        Pathways in Carbon Monoxide Ice at 10 K}",
      journal = {The Astrophysical Journal Supplement Series},
     keywords = {Astrochemistry, Comets: General, ISM: Cosmic Rays, Infrared: ISM, ISM:
        Molecules, Methods: Laboratory, Molecular Processes},
         year = 2006,
        month = Mar,
       volume = {163},
        pages = {184-206},
          doi = {10.1086/499245},
       adsurl = {https://ui.adsabs.harvard.edu/#abs/2006ApJS..163..184J},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Sicilia2012,
       author = {{Sicilia}, D. and {Ioppolo}, S. and {Vindigni}, T. and {Baratta}, G.~A.
        and {Palumbo}, M.~E.},
        title = "{Nitrogen oxides and carbon chain oxides formed after ion irradiation of
        CO:N$_{2}$ ice mixtures}",
      journal = {\aap},
     keywords = {astrochemistry, methods: laboratory, techniques: spectroscopic, ISM:
        molecules, ISM: abundances, molecular processes},
         year = 2012,
        month = Jul,
       volume = {543},
          eid = {A155},
        pages = {A155},
          doi = {10.1051/0004-6361/201219390},
       adsurl = {https://ui.adsabs.harvard.edu/#abs/2012A&A...543A.155S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Fulvio2009,
       author = {{Fulvio}, D. and {Sivaraman}, B. and {Baratta}, G.~A. and {Palumbo},
        M.~E. and {Mason}, N.~J.},
        title = "{Novel measurements of refractive index, density and mid-infrared
        integrated band strengths for solid O2, N2O and NO2 : N2O4
        mixtures}",
      journal = {Spectrochimica Acta Part A: Molecular Spectroscopy},
     keywords = {Nitrous oxide, Nitrogen dioxide, Dinitrogen tetroxide, Infrared
        spectroscopy, Interstellar ices, Band strengths},
         year = 2009,
        month = Jun,
       volume = {72},
        pages = {1007-1013},
          doi = {10.1016/j.saa.2008.12.030},
       adsurl = {https://ui.adsabs.harvard.edu/#abs/2009AcSpA..72.1007F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Pugh1976,
       author = {{Pugh}, Larry A. and {Narahari Rao}, K.},
        title = "{Intensities from Infrared Spectra}",
    booktitle = {Molecular Spectroscopy: Modern Research, Volume II},
         year = 1976,
       editor = {{Rao}, Narahari Rao},
        month = Jan,
        pages = {165},
       adsurl = {https://ui.adsabs.harvard.edu/#abs/1976msmr.conf..165P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Yamada1964,
       author = {{Yamada}, Haruka and {Person}, Willis B.},
        title = "{Absolute Infrared Intensities of the Fundamental Absorption Bands in
        Solid CO$_{2}$ and N$_{2}$O}",
      journal = {\jcp},
         year = 1964,
        month = Oct,
       volume = {41},
        pages = {2478-2487},
          doi = {10.1063/1.1726291},
       adsurl = {https://ui.adsabs.harvard.edu/#abs/1964JChPh..41.2478Y},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Hudgins1993,
       author = {{Hudgins}, D.~M. and {Sandford}, S.~A. and {Allamandola}, L.~J. and
        {Tielens}, A.~G.~G.~M.},
        title = "{Mid- and Far-Infrared Spectroscopy of Ices: Optical Constants and
        Integrated Absorbances}",
      journal = {The Astrophysical Journal Supplement Series},
     keywords = {Absorptivity, Ice, Infrared Spectroscopy, Molecular Absorption, Far
        Infrared Radiation, Infrared Spectra, Organic Compounds,
        Astronomy, LINE: IDENTIFICATION, MOLECULAR DATA},
         year = 1993,
        month = Jun,
       volume = {86},
        pages = {713},
          doi = {10.1086/191796},
       adsurl = {https://ui.adsabs.harvard.edu/#abs/1993ApJS...86..713H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Fayolle2013,
       author = {{Fayolle}, E.~C. and {Bertin}, M. and {Romanzin}, C. and {Poderoso},
        H.~A.~M. and {Philippe}, L. and {Michaut}, X. and {Jeseck}, P.
        and {Linnartz}, H. and {{\"O}berg}, K.~I. and {Fillion}, J. -H.},
        title = "{Wavelength-dependent UV photodesorption of pure N$_{2}$ and O$_{2}$ ices}",
      journal = {\aap},
     keywords = {astrochemistry, ISM: abundances, ISM: molecules, molecular data,
        molecular processes, Astrophysics - Galaxy Astrophysics,
        Astrophysics - Earth and Planetary Astrophysics},
         year = 2013,
        month = Aug,
       volume = {556},
          eid = {A122},
        pages = {A122},
          doi = {10.1051/0004-6361/201321533},
archivePrefix = {arXiv},
       eprint = {1309.4773},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/#abs/2013A&A...556A.122F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Palumbo2006,
       author = {{Palumbo}, M.~E. and {Baratta}, G.~A. and {Collings}, M.~P. and
        {McCoustra}, M.~R.~S.},
        title = "{The profile of the 2140 cm-1 solid CO band on different substrates}",
      journal = {Physical Chemistry Chemical Physics (Incorporating Faraday Transactions)},
         year = 2006,
        month = Jan,
       volume = {8},
        pages = {279-284},
       adsurl = {https://ui.adsabs.harvard.edu/#abs/2006PCCP....8..279P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Gus2014,
       author = {{Cruz-Diaz}, G.~A. and {Mu{\~n}oz Caro}, G.~M. and {Chen}, Y. -J. and
        {Yih}, T. -S.},
        title = "{Vacuum-UV spectroscopy of interstellar ice analogs. I. Absorption cross-
        sections of polar-ice molecules}",
      journal = {\aap},
     keywords = {astrochemistry, ultraviolet: ISM, ISM: molecules, instrumentation:
        spectrographs, methods: laboratory, techniques: photometric,
        Astrophysics - Solar and Stellar Astrophysics, Astrophysics -
        Earth and Planetary Astrophysics, Astrophysics - Astrophysics of
        Galaxies, Physics - Chemical Physics},
         year = 2014,
        month = Feb,
       volume = {562},
          eid = {A119},
        pages = {A119},
          doi = {10.1051/0004-6361/201322140},
archivePrefix = {arXiv},
       eprint = {1405.7797},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/#abs/2014A&A...562A.119C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Gus2014b,
       author = {{Cruz-Diaz}, G.~A. and {Mu{\~n}oz Caro}, G.~M. and {Chen}, Y. -J. and
        {Yih}, T. -S.},
        title = "{Vacuum-UV spectroscopy of interstellar ice analogs. II. Absorption
        cross-sections of nonpolar ice molecules}",
      journal = {\aap},
     keywords = {astrochemistry, methods: laboratory: molecular, methods: laboratory:
        solid state, techniques: spectroscopic, ISM: molecules,
        ultraviolet: ISM, Astrophysics - Solar and Stellar Astrophysics,
        Astrophysics - Earth and Planetary Astrophysics, Condensed
        Matter - Materials Science, Physics - Chemical Physics},
         year = 2014,
        month = Feb,
       volume = {562},
          eid = {A120},
        pages = {A120},
          doi = {10.1051/0004-6361/201322621},
archivePrefix = {arXiv},
       eprint = {1405.7802},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/#abs/2014A&A...562A.120C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Gerakines1995,
       author = {{Gerakines}, P.~A. and {Schutte}, W.~A. and {Greenberg}, J.~M. and {van
        Dishoeck}, E.~F.},
        title = "{The infrared band strengths of H\_2\_O, CO and CO\_2\_ in laboratory
        simulations of astrophysical ice mixtures.}",
      journal = {\aap},
     keywords = {INFRARED: ISM: LINES AND BANDS, ISM: ABUNDANCES, DUST, ISM: MOLECULES,
        MOLECULAR DATA, METHODS: LABORATORY, Astrophysics},
         year = 1995,
        month = Apr,
       volume = {296},
        pages = {810},
archivePrefix = {arXiv},
       eprint = {astro-ph/9409076},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/#abs/1995A&A...296..810G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Stanford1988,
       author = {{Sandford}, S.~A. and {Allamandola}, L.~J. and {Tielens}, A.~G.~G.~M.
        and {Valero}, G.~J.},
        title = "{Laboratory Studies of the Infrared Spectral Properties of CO in
        Astrophysical Ices}",
      journal = {\apj},
     keywords = {Carbon Monoxide, Ice, Infrared Spectra, Interstellar Chemistry,
        Interstellar Matter, Abundance, Line Spectra, Spectral Bands,
        Astrophysics, INFRARED: SPECTRA, LABORATORY SPECTRA, LINE
        IDENTIFICATIONS, MOLECULAR PROCESSES, INTERSTELLAR: GRAINS,
        INTERSTELLAR: MOLECULES, INTERSTELLAR: ABUNDANCES},
         year = 1988,
        month = Jun,
       volume = {329},
        pages = {498},
          doi = {10.1086/166395},
       adsurl = {https://ui.adsabs.harvard.edu/#abs/1988ApJ...329..498S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Pontoppidan2008,
       author = {{Pontoppidan}, Klaus M. and {Boogert}, A.~C.~A. and {Fraser}, Helen J.
        and {van Dishoeck}, Ewine F. and {Blake}, Geoffrey A. and
        {Lahuis}, Fred and {{\"O}berg}, Karin I. and {Evans}, Neal J.,
        II and {Salyk}, Colette},
        title = "{The c2d Spitzer Spectroscopic Survey of Ices around Low-Mass Young
        Stellar Objects. II. CO$_{2}$}",
      journal = {\apj},
     keywords = {astrochemistry, circumstellar matter, dust, extinction, ISM: evolution,
        Astrophysics},
         year = 2008,
        month = May,
       volume = {678},
        pages = {1005-1031},
          doi = {10.1086/533431},
archivePrefix = {arXiv},
       eprint = {0711.4616},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/#abs/2008ApJ...678.1005P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Fayolle2011,
       author = {{Fayolle}, Edith C. and {Bertin}, Mathieu and {Romanzin}, Claire and
        {Michaut}, Xavier and {{\"O}berg}, Karin I. and {Linnartz},
        Harold and {Fillion}, Jean-Hugues},
        title = "{CO Ice Photodesorption: A Wavelength-dependent Study}",
      journal = {\apj},
     keywords = {astrochemistry, ISM: abundances, ISM: molecules, molecular data,
        molecular processes, Astrophysics - Galaxy Astrophysics},
         year = 2011,
        month = Oct,
       volume = {739},
          eid = {L36},
        pages = {L36},
          doi = {10.1088/2041-8205/739/2/L36},
archivePrefix = {arXiv},
       eprint = {1109.0281},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/#abs/2011ApJ...739L..36F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Fillion2014,
       author = {{Fillion}, Jean-Hugues and {Fayolle}, Edith C. and {Michaut}, Xavier and
        {Doronin}, Misha and {Philippe}, Laurent and {Rakovski}, Joseph
        and {Romanzin}, Claire and {Champion}, Noel and {{\"O}berg},
        Karin I. and {Linnartz}, Harold and {Bertin}, Mathieu},
        title = "{Wavelength resolved UV photodesorption and photochemistry of CO2 ice}",
      journal = {Faraday Discussions},
         year = 2014,
        month = Jan,
       volume = {168},
        pages = {533-552},
          doi = {10.1039/C3FD00129F},
       adsurl = {https://ui.adsabs.harvard.edu/#abs/2014FaDi..168..533F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Boogert2011,
       author = {{Boogert}, A.~C.~A. and {Huard}, T.~L. and {Cook}, A.~M. and {Chiar},
        J.~E. and {Knez}, C. and {Decin}, L. and {Blake}, G.~A. and
        {Tielens}, A.~G.~G.~M. and {van Dishoeck}, E.~F.},
        title = "{Ice and Dust in the Quiescent Medium of Isolated Dense Cores}",
      journal = {\apj},
     keywords = {astrochemistry, infrared: ISM, infrared: stars, ISM: abundances, ISM:
        molecules, stars: formation, Astrophysics - Astrophysics of
        Galaxies},
         year = 2011,
        month = Mar,
       volume = {729},
          eid = {92},
        pages = {92},
          doi = {10.1088/0004-637X/729/2/92},
archivePrefix = {arXiv},
       eprint = {1101.2486},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/#abs/2011ApJ...729...92B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Gus2018,
       author = {{Cruz-Diaz}, Gustavo A. and {Mart{\'\i}n-Dom{\'e}nech}, Rafael and
        {Moreno}, Elena and {Mu{\~n}oz Caro}, Guillermo M. and {Chen},
        Yu-Jung},
        title = "{New measurements on water ice photodesorption and product formation
        under ultraviolet irradiation}",
      journal = {\mnras},
     keywords = {methods: laboratory: molecular, protoplanetary discs, ISM: molecules,
        ultraviolet: ISM, Astrophysics - Instrumentation and Methods for
        Astrophysics, Astrophysics - Earth and Planetary Astrophysics},
         year = 2018,
        month = Mar,
       volume = {474},
        pages = {3080-3089},
          doi = {10.1093/mnras/stx2966},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/#abs/2018MNRAS.474.3080C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Gus2016,
       author = {{Cruz-Diaz}, G.~A. and {Mart{\'\i}n-Dom{\'e}nech}, R. and {Mu{\~n}oz
        Caro}, G.~M. and {Chen}, Y. -J.},
        title = "{Negligible photodesorption of methanol ice and active photon-induced
        desorption of its irradiation products}",
      journal = {\aap},
     keywords = {ultraviolet: ISM, astrochemistry, ISM: molecules, methods: laboratory:
        molecular, molecular processes, Astrophysics - Instrumentation
        and Methods for Astrophysics, Astrophysics - Astrophysics of
        Galaxies},
         year = 2016,
        month = Jul,
       volume = {592},
          eid = {A68},
        pages = {A68},
          doi = {10.1051/0004-6361/201526761},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/#abs/2016A&A...592A..68C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Bahr2012,
       author = {{Bahr}, D.~A. and {Baragiola}, R.~A.},
        title = "{Photodesorption of Solid CO$_{2}$ by Ly{\ensuremath{\alpha}}}",
      journal = {\apj},
     keywords = {astrochemistry, methods: laboratory, molecular processes, radiation
        mechanisms: non-thermal},
         year = 2012,
        month = Dec,
       volume = {761},
          eid = {36},
        pages = {36},
          doi = {10.1088/0004-637X/761/1/36},
       adsurl = {https://ui.adsabs.harvard.edu/#abs/2012ApJ...761...36B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Gerakines1999,
       author = {{Gerakines}, P.~A. and {Whittet}, D.~C.~B. and {Ehrenfreund}, P. and
        {Boogert}, A.~C.~A. and {Tielens}, A.~G.~G.~M. and {Schutte},
        W.~A. and {Chiar}, J.~E. and {van Dishoeck}, E.~F. and {Prusti},
        T. and {Helmich}, F.~P. and {de Graauw}, Th.},
        title = "{Observations of Solid Carbon Dioxide in Molecular Clouds with the
        Infrared Space Observatory}",
      journal = {\apj},
     keywords = {ISM: DUST, EXTINCTION, INFRARED: ISM: LINES AND BANDS, ISM: MOLECULES,
        STARS: PRE-MAIN-SEQUENCE, ISM: Dust, Extinction, Infrared: ISM:
        Lines and Bands, ISM: Molecules, Stars: Pre-Main-Sequence},
         year = 1999,
        month = Sep,
       volume = {522},
        pages = {357-377},
          doi = {10.1086/307611},
       adsurl = {https://ui.adsabs.harvard.edu/#abs/1999ApJ...522..357G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Shen2004,
       author = {{Shen}, C.~J. and {Greenberg}, J.~M. and {Schutte}, W.~A. and {van
        Dishoeck}, E.~F.},
        title = "{Cosmic ray induced explosive chemical desorption in dense clouds}",
      journal = {\aap},
     keywords = {ISM: dust, extinction, ISM: cosmic rays, ISM: clouds, ISM: individual:
        objects: L977, IC 5146},
         year = 2004,
        month = Feb,
       volume = {415},
        pages = {203-215},
          doi = {10.1051/0004-6361:20031669},
       adsurl = {https://ui.adsabs.harvard.edu/#abs/2004A&A...415..203S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Ciaravella2016,
       author = {{Ciaravella}, A. and {Chen}, Y. -J. and {Cecchi-Pestellini}, C. and
        {Jim{\'e}nez-Escobar}, A. and {Mu{\~n}oz Caro}, G.~M. and
        {Chuang}, K. -J. and {Huang}, C. -H.},
        title = "{Chemical Evolution of a CO Ice Induced by Soft X-Rays}",
      journal = {\apj},
     keywords = {ISM: molecules, methods: laboratory: molecular, X-rays: ISM},
         year = 2016,
        month = Mar,
       volume = {819},
          eid = {38},
        pages = {38},
          doi = {10.3847/0004-637X/819/1/38},
       adsurl = {https://ui.adsabs.harvard.edu/#abs/2016ApJ...819...38C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Halfen2001,
       author = {{Halfen}, D.~T. and {Apponi}, A.~J. and {Ziurys}, L.~M.},
        title = "{Evaluating the N/O Chemical Network: The Distribution of N$_{2}$O and NO
        in the Sagittarius B2 Complex}",
      journal = {\apj},
     keywords = {Astrochemistry, Galaxy: Center, ISM: Abundances, ISM: Molecules,
        Molecular Processes, Radio Lines: ISM},
         year = 2001,
        month = Nov,
       volume = {561},
        pages = {244-253},
          doi = {10.1086/322770},
       adsurl = {https://ui.adsabs.harvard.edu/#abs/2001ApJ...561..244H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Ziurys1994,
       author = {{Ziurys}, L.~M. and {Apponi}, A.~J. and {Hollis}, J.~M. and {Snyder},
        L.~E.},
        title = "{Detection of Interstellar N 2O: A New Molecule Containing an N-O Bond}",
      journal = {\apj},
     keywords = {Chemical Bonds, Interstellar Gas, Molecular Clouds, Nitrous Oxides,
        Organic Chemistry, Atmospheric Density, Star Formation,
        Telescopes, Temperature, Astrophysics, ISM: MOLECULES, ISM:
        ABUNDANCES, LINE: IDENTIFICATION, GALAXY: CENTER},
         year = 1994,
        month = Dec,
       volume = {436},
        pages = {L181},
          doi = {10.1086/187662},
       adsurl = {https://ui.adsabs.harvard.edu/#abs/1994ApJ...436L.181Z},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Shu1977,
       author = {{Shu}, F.~H.},
        title = "{Self-similar collapse of isothermal spheres and star formation.}",
      journal = {\apj},
     keywords = {Density Distribution, Gravitational Collapse, Isothermal Flow,
        Protostars, Star Formation, Stellar Structure, Critical Point,
        Runge-Kutta Method, Similarity Theorem, Steady State, Stellar
        Envelopes, Astrophysics},
         year = 1977,
        month = Jun,
       volume = {214},
        pages = {488-497},
          doi = {10.1086/155274},
       adsurl = {https://ui.adsabs.harvard.edu/#abs/1977ApJ...214..488S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Shu1987,
       author = {{Shu}, Frank H. and {Adams}, Fred C. and {Lizano}, Susana},
        title = "{Star formation in molecular clouds: observation and theory.}",
      journal = {Annual Review of Astronomy and Astrophysics},
     keywords = {Astrophysics, Molecular Clouds, Star Formation, Stellar Models,
        Astronomical Maps, Binary Stars, Gravitational Collapse,
        Protostars, Star Clusters, Stellar Mass, Astrophysics, Molecular
        Clouds:Star Formation, Pre-Main-Sequence Stars:Star Formation,
        Protostars:Stellar Evolution, Star Formation:Molecular Clouds,
        Star Formation:Pre-Main-Sequence Stars, Stellar
        Evolution:Protostars},
         year = 1987,
        month = Jan,
       volume = {25},
        pages = {23-81},
          doi = {10.1146/annurev.aa.25.090187.000323},
       adsurl = {https://ui.adsabs.harvard.edu/#abs/1987ARA&A..25...23S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Dunham2010,
       author = {{Dunham}, Michael M. and {Evans}, Neal J., II and {Terebey}, Susan and
        {Dullemond}, Cornelis P. and {Young}, Chadwick H.},
        title = "{Evolutionary Signatures in the Formation of Low-Mass Protostars. II.
        Toward Reconciling Models and Observations}",
      journal = {\apj},
     keywords = {stars: formation, stars: low-mass, Astrophysics - Astrophysics of
        Galaxies},
         year = 2010,
        month = Feb,
       volume = {710},
        pages = {470-502},
          doi = {10.1088/0004-637X/710/1/470},
archivePrefix = {arXiv},
       eprint = {0912.5229},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/#abs/2010ApJ...710..470D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@book{huebner1992,
  title={Solar Photo Rates for Planetary Atmospheres and Atmospheric Pollutants},
  author={Huebner, W.F. and Keady, J.J. and Lyon, S.P.},
  isbn={9780792319993},
  lccn={92030457},
  url={https://books.google.es/books?id=4wXgQc1iyHMC},
  year={1992},
  publisher={Springer Netherlands}
}

@ARTICLE{Kim2012,
       author = {{Kim}, Hyo Jeong and {Evans}, Neal J., II and {Dunham}, Michael M. and
        {Lee}, Jeong-Eun and {Pontoppidan}, Klaus M.},
        title = "{CO$_{2}$ Ice Toward Low-luminosity Embedded Protostars: Evidence for
        Episodic Mass Accretion via Chemical History}",
      journal = {\apj},
     keywords = {astrochemistry, ISM: molecules, stars: formation, stars: low-mass,
        stars: protostars, Astrophysics - Solar and Stellar Astrophysics},
         year = 2012,
        month = Oct,
       volume = {758},
          eid = {38},
        pages = {38},
          doi = {10.1088/0004-637X/758/1/38},
archivePrefix = {arXiv},
       eprint = {1208.5797},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/#abs/2012ApJ...758...38K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Loeffler2005,
       author = {{Loeffler}, M.~J. and {Baratta}, G.~A. and {Palumbo}, M.~E. and
        {Strazzulla}, G. and {Baragiola}, R.~A.},
        title = "{CO$_{2}$ synthesis in solid CO by Lyman-{\ensuremath{\alpha}} photons and 200 keV protons}",
      journal = {\aap},
     keywords = {astrochemistry, molecular processes, methods: laboratory, techniques: spectroscopic, ISM: molecules, infrared: ISM},
         year = 2005,
        month = May,
       volume = {435},
        pages = {587-594},
          doi = {10.1051/0004-6361:20042256},
       adsurl = {https://ui.adsabs.harvard.edu/\#abs/2005A&A...435..587L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%AÑADIDOS PARA EL PAPER DEL CH4
%
%
%
%
%
%
%
@ARTICLE{Esmaili2017,
       author = {{Esmaili}, Sasan and {Bass}, Andrew D. and {Cloutier}, Pierre and
        {Sanche}, L{\'e}on and {Huels}, Michael A.},
        title = "{Synthesis of complex organic molecules in simulated methane rich astrophysical ices}",
      journal = {\jcp},
         year = 2017,
        month = Dec,
       volume = {147},
          eid = {224704},
        pages = {224704},
          doi = {10.1063/1.5003898},
       adsurl = {https://ui.adsabs.harvard.edu/\#abs/2017JChPh.147v4704E},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Vasconcelos2017,
       author = {{Vasconcelos}, Fredson de A. and {Pilling}, Sergio and {Rocha}, Will
        R.~M. and {Rothard}, Hermann and {Boduch}, Philippe},
        title = "{Energetic Processing of N$_{2}$:CH$_{4}$ Ices Employing X-Rays and Swift Ions: Implications for Icy Bodies in the Outer Solar System}",
      journal = {\apj},
     keywords = {astrochemistry, methods: laboratory: solid state, planets and satellites: surfaces},
         year = 2017,
        month = Dec,
       volume = {850},
          eid = {174},
        pages = {174},
          doi = {10.3847/1538-4357/aa965f},
       adsurl = {https://ui.adsabs.harvard.edu/\#abs/2017ApJ...850..174V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Abplanalp2017,
       author = {{Abplanalp}, Matthew J. and {Kaiser}, Ralf I.},
        title = "{Implications for Extraterrestrial Hydrocarbon Chemistry: Analysis of Ethylene (C2H4) and D4-Ethylene (C2D4) Ices Exposed to Ionizing Radiation via Combined Infrared Spectroscopy and Reflectron Time-of-flight Mass Spectrometry}",
      journal = {\apj},
     keywords = {astrochemistry, cosmic rays, infrared: general, ISM: molecules, methods: laboratory: solid state, radiation mechanisms: non-thermal},
         year = 2017,
        month = Feb,
       volume = {836},
          eid = {195},
        pages = {195},
          doi = {10.3847/1538-4357/aa5c32},
       adsurl = {https://ui.adsabs.harvard.edu/\#abs/2017ApJ...836..195A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bennett2006,
       author = {{Bennett}, Chris J. and {Jamieson}, Corey S. and {Osamura}, Yoshihiro
        and {Kaiser}, Ralf I.},
        title = "{Laboratory Studies on the Irradiation of Methane in Interstellar, Cometary, and Solar System Ices}",
      journal = {\apj},
     keywords = {Astrochemistry, ISM: Cosmic Rays, ISM: Molecules, Methods: Laboratory, Molecular Processes, Planets and Satellites: General},
         year = 2006,
        month = Dec,
       volume = {653},
        pages = {792-811},
          doi = {10.1086/508561},
       adsurl = {https://ui.adsabs.harvard.edu/\#abs/2006ApJ...653..792B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Moore2003,
       author = {{Moore}, M.~H. and {Hudson}, R.~L.},
        title = "{Infrared study of ion-irradiated N $_{2}$-dominated ices relevant to Triton and Pluto: formation of HCN and HNC}",
      journal = {\icarus},
         year = 2003,
        month = Feb,
       volume = {161},
        pages = {486-500},
          doi = {10.1016/S0019-1035(02)00037-4},
       adsurl = {https://ui.adsabs.harvard.edu/\#abs/2003Icar..161..486M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Hudson2009,
       author = {{Hudson}, R.~L. and {Moore}, M.~H. and {Raines}, L.~L.},
        title = "{Ethane ices in the outer Solar System: Spectroscopy and chemistry}",
      journal = {\icarus},
         year = 2009,
        month = Oct,
       volume = {203},
        pages = {677-680},
          doi = {10.1016/j.icarus.2009.06.026},
       adsurl = {https://ui.adsabs.harvard.edu/\#abs/2009Icar..203..677H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Brunetto2008,
       author = {{Brunetto}, R. and {Caniglia}, G. and {Baratta}, G.~A. and {Palumbo},
        M.~E.},
        title = "{Integrated Near-Infrared Band Strengths of Solid CH$_{4}$ and Its Mixtures with N$_{2}$}",
      journal = {\apj},
     keywords = {astrochemistry, Kuiper Belt, methods: laboratory, techniques: spectroscopic},
         year = 2008,
        month = Oct,
       volume = {686},
        pages = {1480-1485},
          doi = {10.1086/591509},
       adsurl = {https://ui.adsabs.harvard.edu/\#abs/2008ApJ...686.1480B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{deBarros2011,
       author = {{de Barros}, A.~L.~F. and {Bordalo}, V. and {Seperuelo Duarte}, E. and
        {da Silveira}, E.~F. and {Domaracka}, A. and {Rothard}, H. and
        {Boduch}, P.},
        title = "{Cosmic ray impact on astrophysical ices: laboratory studies on heavy ion irradiation of methane}",
      journal = {\aap},
     keywords = {astrochemistry, methods: laboratory, circumstellar matter, ISM: clouds, ISM: molecules},
         year = 2011,
        month = Jul,
       volume = {531},
          eid = {A160},
        pages = {A160},
          doi = {10.1051/0004-6361/201016021},
       adsurl = {https://ui.adsabs.harvard.edu/\#abs/2011A&A...531A.160D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kaiser1998,
       author = {{Kaiser}, R.~I. and {Roessler}, K.},
        title = "{Theoretical and Laboratory Studies on the Interaction of Cosmic-Ray Particles with Interstellar Ices. III. Suprathermal Chemistry-Induced Formation of Hydrocarbon Molecules in Solid Methane (CH$_{4}$), Ethylene (C$_{2}$H$_{4}$), and Acetylene (C$_{2}$H$_{2}$)}",
      journal = {\apj},
     keywords = {ISM: MOLECULES, METHODS: LABORATORY, ISM: COSMIC RAYS, MOLECULAR PROCESSES, ISM: Cosmic Rays, ISM: Molecules, Methods: Laboratory, Molecular Processes},
         year = 1998,
        month = Aug,
       volume = {503},
        pages = {959-975},
          doi = {10.1086/306001},
       adsurl = {https://ui.adsabs.harvard.edu/\#abs/1998ApJ...503..959K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Dartois2005,
       author = {{Dartois}, E. and {Mu{\~n}oz Caro}, G.~M. and {Deboffle}, D. and
        {Montagnac}, G. and {D'Hendecourt}, L.},
        title = "{Ultraviolet photoproduction of ISM dust.  Laboratory characterisation and astrophysical relevance}",
      journal = {\aap},
     keywords = {ISM: dust, extinction, galaxies: ISM, ISM: lines and bands},
         year = 2005,
        month = Mar,
       volume = {432},
        pages = {895-908},
          doi = {10.1051/0004-6361:20042094},
       adsurl = {https://ui.adsabs.harvard.edu/\#abs/2005A&A...432..895D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Hudgins1993,
       author = {{Hudgins}, D.~M. and {Sandford}, S.~A. and {Allamandola}, L.~J. and
        {Tielens}, A.~G.~G.~M.},
        title = "{Mid- and Far-Infrared Spectroscopy of Ices: Optical Constants and Integrated Absorbances}",
      journal = {The Astrophysical Journal Supplement Series},
     keywords = {Absorptivity, Ice, Infrared Spectroscopy, Molecular Absorption, Far Infrared Radiation, Infrared Spectra, Organic Compounds, Astronomy, LINE: IDENTIFICATION, MOLECULAR DATA},
         year = 1993,
        month = Jun,
       volume = {86},
        pages = {713},
          doi = {10.1086/191796},
       adsurl = {https://ui.adsabs.harvard.edu/\#abs/1993ApJS...86..713H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Grundy2016,
       author = {{Grundy}, W.~M. and {Binzel}, R.~P. and {Buratti}, B.~J. and {Cook},
        J.~C. and {Cruikshank}, D.~P. and {Dalle Ore}, C.~M. and
        {Earle}, A.~M. and {Ennico}, K. and {Howett}, C.~J.~A. and
        {Lunsford}, A.~W. and {Olkin}, C.~B. and {Parker}, A.~H. and
        {Philippe}, S. and {Protopapa}, S. and {Quirico}, E. and
        {Reuter}, D.~C. and {Schmitt}, B. and {Singer}, K.~N. and
        {Verbiscer}, A.~J. and {Beyer}, R.~A. and {Buie}, M.~W. and
        {Cheng}, A.~F. and {Jennings}, D.~E. and {Linscott}, I.~R. and
        {Parker}, J. Wm. and {Schenk}, P.~M. and {Spencer}, J.~R. and
        {Stansberry}, J.~A. and {Stern}, S.~A. and {Throop}, H.~B. and
        {Tsang}, C.~C.~C. and {Weaver}, H.~A. and {Weigle}, G.~E. and
        {Young}, L.~A.},
        title = "{Surface compositions across Pluto and Charon}",
      journal = {Science},
     keywords = {GEOCHEM PHYS, PLANET SCI, ONLINE, Astrophysics - Earth and Planetary Astrophysics},
         year = 2016,
        month = Mar,
       volume = {351},
          eid = {aad9189},
        pages = {aad9189},
          doi = {10.1126/science.aad9189},
archivePrefix = {arXiv},
       eprint = {1604.05368},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/\#abs/2016Sci...351.9189G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Cruikshank1993,
       author = {{Cruikshank}, D.~P. and {Roush}, T.~L. and {Owen}, T.~C. and {Geballe},
        T.~R. and {de Bergh}, C. and {Schmitt}, B. and {Brown}, R.~H.
        and {Bartholomew}, M.~J.},
        title = "{Ices on the Surface of Triton}",
      journal = {Science},
     keywords = {Atmospheric Chemistry, Carbon Dioxide, Ice, Satellite Atmospheres, Triton, Astronomical Spectroscopy, Infrared Spectra, Photochemical Reactions, Satellite Surfaces, Lunar and Planetary Exploration; Satellites of Neptune, NEPTUNE, TRITON, SATELLITES, ICE, SURFACE, SPECTROSCOPY, WAVELENGTHS, NEAR-INFRARED, COMPOSITION, NITROGEN, METHANE, CARBON MONOXIDE, SPECTRA, CARBON DIOXIDE, ATMOSPHERE, EARTH-BASED OBSERVATIONS, REFLECTANCE, MODEL, PROCEDURE, PARAMETERS, ABUNDANCE, VOLATILITY, HYPOTHESES, HYDROCARBONS},
         year = 1993,
        month = Aug,
       volume = {261},
        pages = {742-745},
          doi = {10.1126/science.261.5122.742},
       adsurl = {https://ui.adsabs.harvard.edu/\#abs/1993Sci...261..742C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Owen1993,
       author = {{Owen}, T.~C. and {Roush}, T.~L. and {Cruikshank}, D.~P. and {Elliot},
        J.~L. and {Young}, L.~A. and {de Bergh}, C. and {Schmitt}, B.
        and {Geballe}, T.~R. and {Brown}, R.~H. and {Bartholomew}, M.~J.},
        title = "{Surface Ices and the Atmospheric Composition of Pluto}",
      journal = {Science},
     keywords = {Atmospheric Composition, Ice, Planetary Surfaces, Pluto (Planet), Atmospheric Models, Carbon Monoxide, Infrared Spectra, Methane, Solid Nitrogen, Lunar and Planetary Exploration; Pluto, PLUTO, SURFACE, ICE, ATMOSPHERE, COMPOSITION, ABSORPTION, NITROGEN, CARBON MONOXIDE, METHANE, ABUNDANCE, GAS PHASE, SOLID PHASE, NEON, COMPARISON, EARTH-BASED OBSERVATIONS, WAVELENGTHS, SPECTROSCOPY, MODEL, SPECTRA, PRESSURE, GASES, TEMPERATURE, CARBON DIOXIDE, NEPTUNE, SATELLITES, TRITON},
         year = 1993,
        month = Aug,
       volume = {261},
        pages = {745-748},
          doi = {10.1126/science.261.5122.745},
       adsurl = {https://ui.adsabs.harvard.edu/\#abs/1993Sci...261..745O},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Oberg2008,
       author = {{{\"O}berg}, Karin I. and {Boogert}, A.~C. Adwin and {Pontoppidan},
        Klaus M. and {Blake}, Geoffrey A. and {Evans}, Neal J. and
        {Lahuis}, Fred and {van Dishoeck}, Ewine F.},
        title = "{The c2d Spitzer Spectroscopic Survey of Ices around Low-Mass Young Stellar Objects. III. CH$_{4}$}",
      journal = {\apj},
     keywords = {astrochemistry, infrared: ISM, ISM: abundances, ISM: molecules, stars: formation, Astrophysics},
         year = 2008,
        month = May,
       volume = {678},
        pages = {1032-1041},
          doi = {10.1086/533432},
archivePrefix = {arXiv},
       eprint = {0801.1223},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/\#abs/2008ApJ...678.1032O},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{McKay1997,
       author = {{McKay}, Christopher P. and {Martin}, Shuleen Chau and {Griffith},
        Caitlin A. and {Keller}, Richard M.},
        title = "{Temperature Lapse Rate and Methane in Titan's Troposphere}",
      journal = {\icarus},
         year = 1997,
        month = Oct,
       volume = {129},
        pages = {498-505},
          doi = {10.1006/icar.1997.5751},
       adsurl = {https://ui.adsabs.harvard.edu/\#abs/1997Icar..129..498M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Lacy1991,
       author = {{Lacy}, J.~H. and {Carr}, J.~S. and {Evans}, Neal J., II and {Baas}, F.
        and {Achtermann}, J.~M. and {Arens}, J.~F.},
        title = "{Discovery of Interstellar Methane: Observations of Gaseous and Solid CH 4 Absorption toward Young Stars in Molecular Clouds}",
      journal = {\apj},
     keywords = {Cosmic Gases, Interstellar Matter, Methane, Molecular Clouds, Abundance, Early Stars, Infrared Spectra, Solidified Gases, Astrophysics, INFRARED: SPECTRA, INTERSTELLAR: ABUNDANCES, INTERSTELLAR: MOLECULES},
         year = 1991,
        month = Aug,
       volume = {376},
        pages = {556},
          doi = {10.1086/170304},
       adsurl = {https://ui.adsabs.harvard.edu/\#abs/1991ApJ...376..556L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Boogert1996,
       author = {{Boogert}, A.~C.~A. and {Schutte}, W.~A. and {Tielens}, A. and
        {Muñoz Caro}, G. M. and {Whittet}, D.~C.~B. and {Helmich}, F.~P. and {Ehrenfreund}, P.
        and {Wesselius}, P.~R. and {de Graauw}, T. and {Prusti}, T.},
        title = "{Solid methane toward deeply embedded protostars.}",
      journal = {\aap},
     keywords = {ISM: DUST, EXTINCTION, ISM: MOLECULES, ISM: ABUNDANCES, INFRARED: ISM: LINES AND BANDS, STARS: INDIVIDUAL: NGC 7538 IRS9, STARS: INDIVIDUAL: W 33A},
         year = 1996,
        month = Nov,
       volume = {315},
        pages = {L377-L380},
       adsurl = {https://ui.adsabs.harvard.edu/\#abs/1996A&A...315L.377B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Dartois2004,
       author = {{Dartois}, E. and {Mu{\~n}oz Caro}, G.~M. and {Deboffle}, D. and
        {d'Hendecourt}, L.},
        title = "{Diffuse interstellar medium organic polymers. Photoproduction of the 3.4, 6.85 and 7.25 {\ensuremath{\mu}}m features}",
      journal = {\aap},
     keywords = {ISM: dust, extinction, lines and bands},
         year = 2004,
        month = Aug,
       volume = {423},
        pages = {L33-L36},
          doi = {10.1051/0004-6361:200400032},
       adsurl = {https://ui.adsabs.harvard.edu/\#abs/2004A&A...423L..33D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Hudson1997,
       author = {{Hudson}, R.~L. and {Moore}, M.~H.},
        title = "{NOTE: Hydrocarbon Radiation Chemistry in Ices of Cometary Relevance}",
      journal = {\icarus},
         year = 1997,
        month = Mar,
       volume = {126},
        pages = {233-235},
          doi = {10.1006/icar.1997.5678},
       adsurl = {https://ui.adsabs.harvard.edu/\#abs/1997Icar..126..233H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Pilling2009,
       author = {{Pilling}, Sergio and {Andrade}, Diana P.~P. and {Neto}, {\'A}lvaro C.
        and {Rittner}, Roberto and {Naves de Brito}, Arnaldo},
        title = "{DNA Nucleobase Synthesis at Titan Atmosphere Analog by Soft X-rays}",
      journal = {Journal of Physical Chemistry A},
         year = 2009,
        month = Jun,
       volume = {113},
        pages = {11161-11166},
          doi = {10.1021/jp902824v},
       adsurl = {https://ui.adsabs.harvard.edu/\#abs/2009JPCA..11311161P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bohn1994,
       author = {{Bohn}, Robert B. and {Sandford}, Scott A. and {Allamandola}, Louis J. and
         {Cruikshank}, Dale P.},
        title = "{Infrared Spectroscopy of Triton and Pluto Ice Analogs: The Case for Saturated Hydrocarbons}",
      journal = {\icarus},
     keywords = {Analogs, Ice, Infrared Spectra, Nitrogen, Photochemical Reactions, Pluto (Planet), Triton, Absorption Spectra, Abundance, Alkanes, Astronomical Models, Infrared Spectroscopy, Planetary Surfaces, Satellite Surfaces, Lunar and Planetary Exploration},
         year = "1994",
        month = "Sep",
       volume = {111},
        pages = {151-173},
          doi = {10.1006/icar.1994.1138},
       adsurl = {https://ui.adsabs.harvard.edu/\#abs/1994Icar..111..151B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Guille2002,
       author = {{Mu{\~n}oz Caro}, G.~M. and {Meierhenrich}, U.~J. and {Schutte}, W.~A. and
         {Barbier}, B. and {Arcones Segovia}, A. and {Rosenbauer}, H. and
         {Thiemann}, W.~H. -P. and {Brack}, A. and {Greenberg}, J.~M.},
        title = "{Amino acids from ultraviolet irradiation of interstellar ice analogues}",
      journal = {\nat},
         year = "2002",
        month = "Mar",
       volume = {416},
        pages = {403-406},
          doi = {10.1038/416403a},
       adsurl = {https://ui.adsabs.harvard.edu/\#abs/2002Natur.416..403M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Rakhovskaia1995,
       author = {{Rakhovskaia}, O. and {Wiethoff}, P. and {Feulner}, P.},
        title = "{Thresholds for electron stimulated desorption of neutral molecules from solid N $_{2}$, CO, O $_{2}$ and NO}",
      journal = {Nuclear Instruments and Methods in Physics Research B},
         year = "1995",
        month = "Jun",
       volume = {101},
        pages = {169-173},
          doi = {10.1016/0168-583X(95)00296-0},
       adsurl = {https://ui.adsabs.harvard.edu/\#abs/1995NIMPB.101..169R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{MD2018,
       author = {{Mart{\'\i}n-Dom{\'e}nech}, R. and {Cruz-D{\'\i}az}, G.~A. and
         {Mu{\~n}oz Caro}, G.~M.},
        title = "{UV photoprocessing of NH$_{3}$ ice: photon-induced desorption mechanisms}",
      journal = {\mnras},
     keywords = {methods: laboratory: molecular, ISM: clouds, ISM: molecules, Astrophysics - Astrophysics of Galaxies, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = "2018",
        month = "Jan",
       volume = {473},
        pages = {2575-2582},
          doi = {10.1093/mnras/stx2510},
archivePrefix = {arXiv},
       eprint = {1710.06467},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/\#abs/2018MNRAS.473.2575M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
} 

@article{Lin2014,
author = {Lin, Meng-Yeh and Lo, Jen-Iu and Lu, Hsiao-Chi and Chou, Sheng-Lung and Peng, Yu-Chain and Cheng, Bing-Ming and Ogilvie, J. F.},
title = {Vacuum-Ultraviolet Photolysis of Methane at 3 K: Synthesis of Carbon Clusters up to C20},
journal = {The Journal of Physical Chemistry A},
volume = {118},
number = {19},
pages = {3438-3449},
year = {2014},
doi = {10.1021/jp502637r},
URL = { 
        https://doi.org/10.1021/jp502637r
    
},
eprint = { 
        https://doi.org/10.1021/jp502637r
    
}

}

@ARTICLE{Dupuy2017,
   author = {{Dupuy}, R. and {Bertin}, M. and {F{\'e}raud}, G. and {Michaut}, X. and 
	{Jeseck}, P. and {Doronin}, M. and {Philippe}, L. and {Romanzin}, C. and 
	{Fillion}, J.-H.},
    title = "{Spectrally-resolved UV photodesorption of CH$_{4}$ in pure and layered ices}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1704.05398},
 keywords = {astrochemistry, ISM: abundances, ISM: molecules, molecular processes, methods: laboratory: solid state},
     year = 2017,
    month = jul,
   volume = 603,
      eid = {A61},
    pages = {A61},
      doi = {10.1051/0004-6361/201730772},
   adsurl = {http://adsabs.harvard.edu/abs/2017A%26A...603A..61D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Guille2001,
author = {Mu\~noz Caro, G and Ruiterkamp, Richard and A. Schutte, W and Greenberg, J.M. and Mennella, V},
year = {2001},
month = {02},
pages = {},
title = {UV photodestruction of CH bonds and the evolution of the 3.4 mu m feature carrier. I. The case of aliphatic and aromatic molecular species},
volume = {367},
journal = {Astronomy and Astrophysics, 367, 347 - 354 (2001)},
doi = {10.1051/0004-6361:20000341}
}

@ARTICLE{Baratta2002,
   author = {{Baratta}, G.~A. and {Leto}, G. and {Palumbo}, M.~E.},
    title = "{A comparison of ion irradiation and UV photolysis of CH$_{4}$ and CH$_{3}$OH}",
  journal = {\aap},
 keywords = {ASTROCHEMISTRY, MOLECULAR PROCESSES, METHODS: LABORATORY, TECHNIQUES: SPECTROSCOPIC, ISM: MOLECULES},
     year = 2002,
    month = mar,
   volume = 384,
    pages = {343-349},
      doi = {10.1051/0004-6361:20011835},
   adsurl = {https://ui.adsabs.harvard.edu/abs/2002A%26A...384..343B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Oberg2011,
   author = {{{\"O}berg}, K.~I. and {Boogert}, A.~C.~A. and {Pontoppidan}, K.~M. and 
	{van den Broek}, S. and {van Dishoeck}, E.~F. and {Bottinelli}, S. and 
	{Blake}, G.~A. and {Evans}, II, N.~J.},
    title = "{The Spitzer Ice Legacy: Ice Evolution from Cores to Protostars}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1107.5825},
 keywords = {astrochemistry, circumstellar matter, infrared: ISM, ISM: abundances, ISM: lines and bands, ISM: molecules, molecular processes, stars: formation},
     year = 2011,
    month = oct,
   volume = 740,
      eid = {109},
    pages = {109},
      doi = {10.1088/0004-637X/740/2/109},
   adsurl = {https://ui.adsabs.harvard.edu/abs/2011ApJ...740..109O},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Mumma1996,
   author = {{Mumma}, M.~J. and {Disanti}, M.~A. and {dello Russo}, N. and 
	{Fomenkova}, M. and {Magee-Sauer}, K. and {Kaminski}, C.~D. and 
	{Xie}, D.~X.},
    title = "{Detection of Abundant Ethane and Methane, Along with Carbon Monoxide and Water, in Comet C/1996 B2 Hyakutake: Evidence for Interstellar Origin}",
  journal = {Science},
     year = 1996,
    month = may,
   volume = 272,
    pages = {1310-1314},
      doi = {10.1126/science.272.5266.1310},
   adsurl = {https://ui.adsabs.harvard.edu/abs/1996Sci...272.1310M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Oberg2010,
   author = {{{\"O}berg}, K.~I. and {van Dishoeck}, E.~F. and {Linnartz}, H. and 
	{Andersson}, S.},
    title = "{The Effect of H$_{2}$O on Ice Photochemistry}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1006.2190},
 keywords = {astrochemistry, circumstellar matter, ISM: molecules, methods: laboratory, molecular data, molecular processes},
     year = 2010,
    month = aug,
   volume = 718,
    pages = {832-840},
      doi = {10.1088/0004-637X/718/2/832},
   adsurl = {https://ui.adsabs.harvard.edu/abs/2010ApJ...718..832O},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Luna2017,
   author = {{Luna}, R. and {Luna-Ferr{\'a}ndiz}, R. and {Mill{\'a}n}, C. and 
	{Domingo}, M. and {Mu{\~n}oz Caro}, G.~M. and {Santonja}, C. and 
	{Satorre}, M.~{\'A}.},
    title = "{A Fast, Direct Procedure to Estimate the Desorption Energy for Various Molecular Ices of Astrophysical Interest}",
  journal = {\apj},
 keywords = {ISM: kinematics and dynamics, ISM: molecules, methods: laboratory: molecular, methods: laboratory: solid state},
     year = 2017,
    month = jun,
   volume = 842,
      eid = {51},
    pages = {51},
      doi = {10.3847/1538-4357/aa7562},
   adsurl = {https://ui.adsabs.harvard.edu/abs/2017ApJ...842...51L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Cristobal2019,
   author = {{Gonz{\'a}lez D{\'{\i}}az}, C. and {Carrascosa de Lucas}, H. and 
	{Aparicio}, S. and {Mu{\~n}oz Caro}, G.~M. and {Sie}, N.-E. and 
	{Hsiao}, L.-C. and {Cazaux}, S. and {Chen}, Y.-J.},
    title = "{Accretion and photodesorption of CO ice as a function of the incident angle of deposition}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1905.02426},
 keywords = {methods: laboratory, techniques: spectroscopic, ISM: molecules, ultraviolet: ISM},
     year = 2019,
    month = jul,
   volume = 486,
    pages = {5519-5525},
      doi = {10.1093/mnras/stz1223},
   adsurl = {https://ui.adsabs.harvard.edu/abs/2019MNRAS.486.5519G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{VanHemert2015,
       author = {{van Hemert}, Marc C. and {Takahashi}, Junko and
         {van Dishoeck}, Ewine F.},
        title = "{Molecular Dynamics Study of the Photodesorption of CO Ice}",
      journal = {Journal of Physical Chemistry A},
         year = "2015",
        month = "Jun",
       volume = {119},
       number = {24},
        pages = {6354-6369},
          doi = {10.1021/acs.jpca.5b02611},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015JPCA..119.6354V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Andersson2008,
       author = {{Andersson}, S. and {van Dishoeck}, E.~F.},
        title = "{Photodesorption of water ice. A molecular dynamics study}",
      journal = {\aap},
     keywords = {astrochemistry, molecular data, ISM: molecules, Astrophysics},
         year = "2008",
        month = "Dec",
       volume = {491},
       number = {3},
        pages = {907-916},
          doi = {10.1051/0004-6361:200810374},
archivePrefix = {arXiv},
       eprint = {0810.1916},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008A&A...491..907A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bertin2016,
       author = {{Bertin}, Mathieu and {Romanzin}, Claire and {Doronin}, Mikhail and
         {Philippe}, Laurent and {Jeseck}, Pascal and {Ligterink}, Niels and
         {Linnartz}, Harold and {Michaut}, Xavier and {Fillion}, Jean-Hugues},
        title = "{UV Photodesorption of Methanol in Pure and CO-rich Ices: Desorption Rates of the Intact Molecule and of the Photofragments}",
      journal = {\apjl},
     keywords = {astrochemistry, ISM: abundances, ISM: molecules, molecular processes, Astrophysics - Astrophysics of Galaxies},
         year = "2016",
        month = "Feb",
       volume = {817},
       number = {2},
          eid = {L12},
        pages = {L12},
          doi = {10.3847/2041-8205/817/2/L12},
archivePrefix = {arXiv},
       eprint = {1601.07027},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016ApJ...817L..12B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{BingMing2004,
author = {Lu, Hsiao-Chi and Chen, Hong-Kai and Cheng, Bing-Ming},
year = {2004},
month = {11},
pages = {5965-7},
title = {Analysis of C2H4 in C2H6 and C2H5D with VUV absorption spectroscopy and a method to remove C2H4 from C2H6 and C2H5D},
volume = {76},
journal = {Analytical chemistry},
doi = {10.1021/ac0494679}
}


@ARTICLE{Young2018,
       author = {{Young}, Leslie A. and {Kammer}, Joshua A. and {Steffl}, Andrew J. and
         {Gladstone}, G. Randall and {Summers}, Michael E. and
         {Strobel}, Darrell F. and {Hinson}, David P. and {Stern}, S. Alan and
         {Weaver}, Harold A. and {Olkin}, Catherine B. and {Ennico}, Kimberly and
         {McComas}, David J. and {Cheng}, Andrew F. and {Gao}, Peter and
         {Lavvas}, Panayotis and {Linscott}, Ivan R. and {Wong}, Michael L. and
         {Yung}, Yuk L. and {Cunningham}, Nathanial and {Davis}, Michael and
         {Parker}, Joel Wm. and {Schindhelm}, Eric and {Siegmund}, Oswald H.~W. and
         {Stone}, John and {Retherford}, Kurt and {Versteeg}, Maarten},
        title = "{Structure and composition of Pluto's atmosphere from the New Horizons solar ultraviolet occultation}",
      journal = {\icarus},
     keywords = {Pluto, atmosphere, Atmospheres, structure, Occultations, Ultraviolet observations, Triton, KBO atmospheres, Astrophysics - Earth and Planetary Astrophysics},
         year = "2018",
        month = "Jan",
       volume = {300},
        pages = {174-199},
          doi = {10.1016/j.icarus.2017.09.006},
archivePrefix = {arXiv},
       eprint = {1704.01511},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018Icar..300..174Y},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Satorre2008,
       author = {{Satorre}, M. {\'A}. and {Domingo}, M. and {Mill{\'a}n}, C. and
         {Luna}, R. and {Vilaplana}, R. and {Santonja}, C.},
        title = "{Density of CH$_{4}$, N$_{2}$ and CO$_{2}$ ices at different temperatures of deposition}",
      journal = {\planss},
         year = "2008",
        month = "Nov",
       volume = {56},
       number = {13},
        pages = {1748-1752},
          doi = {10.1016/j.pss.2008.07.015},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008P&SS...56.1748S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Hudson2015,
       author = {{Hudson}, R.~L. and {Gerakines}, P.~A. and {Loeffler}, M.~J.},
        title = "{Activation of weak IR fundamentals of two species of astrochemical interest in the Tdpoint group - the importance of amorphous ices}",
      journal = {Physical Chemistry Chemical Physics (Incorporating Faraday Transactions)},
         year = "2015",
        month = "Jan",
       volume = {17},
       number = {19},
        pages = {12545-12552},
          doi = {10.1039/C5CP00975H},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015PCCP...1712545H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Abplanalp2018PCCP...20.5435A,
       author = {{Abplanalp}, Matthew J. and {Jones}, Brant M. and {Kaiser}, Ralf I.},
        title = "{Untangling the methane chemistry in interstellar and solar system ices toward ionizing radiation: a combined infrared and reflectron time-of-flight analysis}",
      journal = {Physical Chemistry Chemical Physics (Incorporating Faraday Transactions)},
         year = "2018",
        month = "Feb",
       volume = {20},
        pages = {5435-5468},
          doi = {10.1039/C7CP05882A},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018PCCP...20.5435A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Lo2015MNRAS.451..159L,
       author = {{Lo}, Jen-Iu and {Lin}, Meng-Yeh and {Peng}, Yu-Chain and
         {Chou}, Sheng-Lung and {Lu}, Hsiao-Chi and {Cheng}, Bing-Ming and
         {Ogilvie}, J.~F.},
        title = "{Far-ultraviolet photolysis of solid methane}",
      journal = {\mnras},
         year = "2015",
        month = "Jul",
       volume = {451},
       number = {1},
        pages = {159-166},
          doi = {10.1093/mnras/stv935},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015MNRAS.451..159L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Magee-Sauer2008,
       author = {{Magee-Sauer}, Karen and {Mumma}, Michael J. and {DiSanti}, Michael A. and
         {Dello Russo}, Neil and {Gibb}, Erika L. and {Bonev}, Boncho P. and
         {Villanueva}, G.~L.},
        title = "{The organic composition of Comet C/2001 A2 (LINEAR). I. Evidence for an unusual organic chemistry}",
      journal = {\icarus},
         year = "2008",
        month = "Mar",
       volume = {194},
       number = {1},
        pages = {347-356},
          doi = {10.1016/j.icarus.2007.10.006},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008Icar..194..347M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bossa2015PCCP...1717346B,
       author = {{Bossa}, J. -B. and {Paardekooper}, D.~M. and {Isokoski}, K. and
         {Linnartz}, H.},
        title = "{Methane ice photochemistry and kinetic study using laser desorption time-of-flight mass spectrometry at 20 K}",
      journal = {Physical Chemistry Chemical Physics (Incorporating Faraday Transactions)},
         year = "2015",
        month = "Jan",
       volume = {17},
       number = {26},
        pages = {17346-17354},
          doi = {10.1039/C5CP00578G},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015PCCP...1717346B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Moore1998Icar..135..518M,
       author = {{Moore}, M.~H. and {Hudson}, R.~L.},
        title = "{Infrared Study of Ion-Irradiated Water-Ice Mixtures with Hydrocarbons Relevant to Comets}",
      journal = {\icarus},
         year = "1998",
        month = "Oct",
       volume = {135},
       number = {2},
        pages = {518-527},
          doi = {10.1006/icar.1998.5996},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1998Icar..135..518M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{d'hendecourt1996AA...315L.365D,
       author = {{D'Hendecourt}, L. and {Jourdain de Muizon}, M. and {Dartois}, E. and
         {Breitfellner}, M. and {Ehrenfreund}, P. and {Benit}, J. and
         {Boulanger}, F. and {Puget}, J.~L. and {Habing}, H.~J.},
        title = "{ISO-SWS observations of solid state features towards RAFGL 7009S.}",
      journal = {\aap},
     keywords = {ISM: MOLECULES, ISM: ABUNDANCES, ISM: DUST, EXTINCTION, ISM: INDIVIDUAL: RAFGL 7009S},
         year = "1996",
        month = "Nov",
       volume = {315},
        pages = {L365-L368},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1996A&A...315L.365D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Dartois2005SSRv..119..293D,
       author = {{Dartois}, Emmanuel},
        title = "{The Ice Survey Opportunity of ISO}",
      journal = {\ssr},
     keywords = {ices, dust, infrared absorption},
         year = "2005",
        month = "Aug",
       volume = {119},
       number = {1-4},
        pages = {293-310},
          doi = {10.1007/s11214-005-8059-9},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2005SSRv..119..293D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Boogert2015ARA&A..53..541B,
       author = {{Boogert}, A.~C. Adwin and {Gerakines}, Perry A. and
         {Whittet}, Douglas C.~B.},
        title = "{Observations of the icy universe.}",
      journal = {\araa},
     keywords = {Astrophysics - Astrophysics of Galaxies, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = "2015",
        month = "Aug",
       volume = {53},
        pages = {541-581},
          doi = {10.1146/annurev-astro-082214-122348},
archivePrefix = {arXiv},
       eprint = {1501.05317},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015ARA&A..53..541B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Gredel1989ApJ...347..289G,
       author = {{Gredel}, R. and {Lepp}, S. and {Dalgarno}, A. and {Herbst}, E.},
        title = "{Cosmic-Ray--induced Photodissociation and Photoionization Rates of Interstellar Molecules}",
      journal = {\apj},
     keywords = {Cosmic Rays, Interstellar Matter, Photodissociation, Photoionization, Electron Impact, Emission Spectra, Hydrogen, Molecules, Ultraviolet Radiation, Astrophysics, COSMIC RAYS: GENERAL, INTERSTELLAR: MOLECULES},
         year = "1989",
        month = "Dec",
       volume = {347},
        pages = {289},
          doi = {10.1086/168117},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1989ApJ...347..289G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Wu2012ApJ...746..175W,
       author = {{Wu}, Yu-Jong and {Wu}, C.~Y. Robert and {Chou}, Sheng-Lung and
         {Lin}, Meng-Yeh and {Lu}, Hsiao-Chi and {Lo}, Jen-Iu and
         {Cheng}, Bing-Ming},
        title = "{Spectra and Photolysis of Pure Nitrogen and Methane Dispersed in Solid Nitrogen with Vacuum-Ultraviolet Light}",
      journal = {\apj},
     keywords = {astrochemistry, infrared: ISM, ISM: molecules, methods: laboratory, molecular processes},
         year = "2012",
        month = "Feb",
       volume = {746},
       number = {2},
          eid = {175},
        pages = {175},
          doi = {10.1088/0004-637X/746/2/175},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012ApJ...746..175W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{d'Hendecourt1986AA...158..119D,
       author = {{D'Hendecourt}, L.~B. and {Allamandola}, L.~J. and {Grim}, R.~J.~A. and
         {Greenberg}, J.~M.},
        title = "{Time-dependent chemistry in dense molecular clouds. II. Ultraviolet photoprocessing and infrared spectroscopy of grain mantles.}",
      journal = {\aap},
     keywords = {Cosmic Dust, Infrared Astronomy, Interstellar Chemistry, Molecular Clouds, Photolysis, Ultraviolet Radiation, Absorption Spectra, Ice, Infrared Spectra, Photodissociation, Solid Phases, Time Dependence, Vapor Phases, Astrophysics},
         year = "1986",
        month = "Apr",
       volume = {158},
        pages = {119-134},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1986A&A...158..119D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}







%%%%%%%%%%%% RELACIONADOS CON LA SÍNTESIS DEL HMT, MÁS PREBIÓTICO
@ARTICLE{Vinogradoff2013,
       author = {{Vinogradoff}, V. and {Fray}, N. and {Duvernay}, F. and {Briani}, G. and
         {Danger}, G. and {Cottin}, H. and {Theul{\'e}}, P. and {Chiavassa}, T.},
        title = "{Importance of thermal reactivity for hexamethylenetetramine formation from simulated interstellar ices}",
      journal = {\aap},
     keywords = {astrochemistry, ISM: molecules},
         year = "2013",
        month = "Mar",
       volume = {551},
          eid = {A128},
        pages = {A128},
          doi = {10.1051/0004-6361/201220870},
       adsurl = {https://ui.adsabs.harvard.edu/\#abs/2013A&A...551A.128V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Hulett1971,
   author = {{Hulett}, H.~R. and {Wolman}, Y. and {Miller}, S.~L. and {Ibanez}, J. and 
	{Oro}, J. and {Fox}, S.~W. and {Windsor}, C.~R.},
    title = "{Formaldehyde and Ammonia as Precursors to Prebiotic Amino Acids}",
  journal = {Science},
     year = 1971,
    month = dec,
   volume = 174,
    pages = {1038-1041},
      doi = {10.1126/science.174.4013.1038},
   adsurl = {https://ui.adsabs.harvard.edu/abs/1971Sci...174.1038H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Vinogradoff2012,
   author = {{Vinogradoff}, V. and {Rimola}, A. and {Duvernay}, F. and {Danger}, G. and 
	{Theul{\'e}}, P. and {Chiavassa}, T.},
    title = "{The mechanism of hexamethylenetetramine (HMT) formation in the solid state at low temperature}",
  journal = {Physical Chemistry Chemical Physics (Incorporating Faraday Transactions)},
     year = 2012,
   volume = 14,
    pages = {12309},
      doi = {10.1039/C2CP41963G},
   adsurl = {https://ui.adsabs.harvard.edu/abs/2012PCCP...1412309V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Vinogradoff2011,
       author = {{Vinogradoff}, V. and {Duvernay}, F. and {Danger}, G. and
         {Theul{\'e}}, P. and {Chiavassa}, T.},
        title = "{New insight into the formation of hexamethylenetetramine (HMT) in interstellar and cometary ice analogs}",
      journal = {\aap},
     keywords = {astrochemistry, ISM: molecules, methods: laboratory},
         year = "2011",
        month = "Jun",
       volume = {530},
          eid = {A128},
        pages = {A128},
          doi = {10.1051/0004-6361/201116688},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011A&A...530A.128V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Vinogradoff2012b,
       author = {{Vinogradoff}, V. and {Duvernay}, F. and {Danger}, G. and
         {Theul{\'e}}, P. and {Borget}, F. and {Chiavassa}, T.},
        title = "{Formaldehyde and methylamine reactivity in interstellar ice analogues as a source of molecular complexity at low temperature}",
      journal = {\aap},
     keywords = {astrochemistry, molecular processes, methods: laboratory, ISM: molecules},
         year = "2013",
        month = "Jan",
       volume = {549},
          eid = {A40},
        pages = {A40},
          doi = {10.1051/0004-6361/201219974},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013A&A...549A..40V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bernstein1995,
       author = {{Bernstein}, Max P. and {Sandford}, Scott A. and {Allamand
        ola}, Louis J. and {Chang}, Sherwood and {Scharberg}, Maureen A.},
        title = "{Organic Compounds Produced by Photolysis of Realistic Interstellar and Cometary Ice Analogs Containing Methanol}",
      journal = {\apj},
     keywords = {ISM: DUST, EXTINCTION, INFRARED: ISM: LINES AND BANDS, ISM: MOLECULES, MOLECULAR PROCESSES},
         year = "1995",
        month = "Nov",
       volume = {454},
        pages = {327},
          doi = {10.1086/176485},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1995ApJ...454..327B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Ogura1989,
title = "Photolysis of CH4NH3H2O mixture: formation of methylamine and ethylenediamine",
journal = "Journal of Photochemistry and Photobiology A: Chemistry",
volume = "49",
number = "1",
pages = "53 - 61",
year = "1989",
issn = "1010-6030",
doi = "https://doi.org/10.1016/1010-6030(89)87105-9",
url = "http://www.sciencedirect.com/science/article/pii/1010603089871059",
author = "K. Ogura and C.T. Migita and T. Yamada",
abstract = "The photolysis of the mixture CH4NH3H2O was performed with a low pressure mercury lamp at 100 °C and atmospheric pressure. Of the products, the major nitrogen-containing compounds were methylamine and ethylenediamine; the maximum selectivity of the two amines exceeded 99% in the mol per cent of N-containing products. The other products were methanol, ethane and hydrogen, but the formation of methanol and ethane decreased rapidly with an increase in the amount of added ammonia. This was attributed to the preferential reactivity of methyl radicals with NH2 rather than with OH and/or CH3. The formation rates of NH2, CH3NH2 and NH2C2H4NH2 are discussed."
}

@article{Gardner1982,
author = {Gardner, Edward P. and McNesby, James R.},
title = {Vacuum-ultraviolet photolysis of methylamine},
journal = {The Journal of Physical Chemistry},
volume = {86},
number = {14},
pages = {2646-2651},
year = {1982},
doi = {10.1021/j100211a019},
}

@ARTICLE{Herbst1985,
       author = {{Herbst}, E.},
        title = "{The rate of the radiative association reaction between CH3(+) and NH3 and its implications for interstellar chemistry}",
      journal = {\apj},
     keywords = {Ammonia, Association Reactions, Interstellar Chemistry, Methyl Compounds, Activation Energy, Molecular Clouds, Quantum Numbers, Astrophysics},
         year = "1985",
        month = "May",
       volume = {292},
        pages = {484-486},
          doi = {10.1086/163179},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1985ApJ...292..484H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Oba2017ApJ...849..122O,
       author = {{Oba}, Yasuhiro and {Takano}, Yoshinori and {Naraoka}, Hiroshi and
         {Kouchi}, Akira and {Watanabe}, Naoki},
        title = "{Deuterium Fractionation upon the Formation of Hexamethylenetetramines through Photochemical Reactions of Interstellar Ice Analogs Containing Deuterated Methanol Isotopologues}",
      journal = {\apj},
     keywords = {astrochemistry, ISM: clouds, solid state: volatile, ultraviolet: ISM},
         year = "2017",
        month = "Nov",
       volume = {849},
       number = {2},
          eid = {122},
        pages = {122},
          doi = {10.3847/1538-4357/aa8ea5},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017ApJ...849..122O},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Butscher2016A&A...593A..60B,
       author = {{Butscher}, Teddy and {Duvernay}, Fabrice and {Danger}, Gr{\'e}goire and
         {Chiavassa}, Thierry},
        title = "{Radical-induced chemistry from VUV photolysis of interstellar ice analogues containing formaldehyde}",
      journal = {\aap},
     keywords = {astrochemistry, molecular data, methods: laboratory: solid state, ISM: molecules},
         year = "2016",
        month = "Sep",
       volume = {593},
          eid = {A60},
        pages = {A60},
          doi = {10.1051/0004-6361/201628258},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016A&A...593A..60B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@Article{Wang2016,
author="WANG, NANA
and TAN, XIAOJUN
and WANG, WEIHUA
and WANG, FANGFANG
and LI, PING",
title="Theoretical insights into the cycloaddition reaction mechanism between ketenimine and methyleneimine: An alternative approach to the formation of pyrazole and imidazole",
journal="Journal of Chemical Sciences",
year="2016",
month="Feb",
day="01",
volume="128",
number="2",
pages="279--285",
abstract="The cycloaddition reaction mechanism between interstellar molecules, ketenimine and methyleneimine, has been systematically investigated employing the second-order M{\o}ller-Plesset perturbation theory (MP2) method in order to better understand the reactivity of nitrogenous cumulene ketenimine with the C =N double bond compound methyleneimine. Geometry optimizations and vibrational analyses have been performed for the stationary points on the potential energy surfaces of the system. Calculations show that five-membered cyclic carbene intermediates could be produced through pericyclic reaction processes between ketenimine and methyleneimine. Through the subsequent hydrogen transfer processes, carbene intermediates can be isomerized to the pyrazole and imidazole compounds, respectively. The present study is helpful to understand the formation of prebiotic species in interstellar space.",
issn="0973-7103",
doi="10.1007/s12039-015-1028-2",
url="https://doi.org/10.1007/s12039-015-1028-2"
}

@ARTICLE{Theule2011AA...534A..64T,
       author = {{Theule}, P. and {Borget}, F. and {Mispelaer}, F. and {Danger}, G. and
         {Duvernay}, F. and {Guillemin}, J.~C. and {Chiavassa}, T.},
        title = "{Hydrogenation of solid hydrogen cyanide HCN and methanimine CH$_{2}$NH at low temperature}",
      journal = {\aap},
     keywords = {astrochemistry, ISM: molecules, molecular processes},
         year = "2011",
        month = "Oct",
       volume = {534},
          eid = {A64},
        pages = {A64},
          doi = {10.1051/0004-6361/201117494},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011A&A...534A..64T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Zhu2019PCCP...21.1952Z,
       author = {{Zhu}, Cheng and {Frigge}, Robert and {Turner}, Andrew M. and
         {Abplanalp}, Matthew J. and {Sun}, Bing-Jian and {Chen}, Yue-Lin and
         {Chang}, Agnes H.~H. and {Kaiser}, Ralf I.},
        title = "{A vacuum ultraviolet photoionization study on the formation of methanimine (CH2NH) and ethylenediamine (NH2CH2CH2NH2) in low temperature interstellar model ices exposed to ionizing radiation}",
      journal = {Physical Chemistry Chemical Physics (Incorporating Faraday Transactions)},
         year = "2019",
        month = "Jan",
       volume = {21},
       number = {4},
        pages = {1952-1962},
          doi = {10.1039/C8CP06002A},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019PCCP...21.1952Z},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Chaabouni2018AA...612A..47C,
       author = {{Chaabouni}, H. and {Diana}, S. and {Nguyen}, T. and {Dulieu}, F.},
        title = "{Thermal desorption of formamide and methylamine from graphite and amorphous water ice surfaces}",
      journal = {\aap},
     keywords = {methods: laboratory: molecular, molecular processes, astrochemistry, techniques: spectroscopic, ISM: molecules, dust, extinction, Astrophysics - Astrophysics of Galaxies, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = "2018",
        month = "Apr",
       volume = {612},
          eid = {A47},
        pages = {A47},
          doi = {10.1051/0004-6361/201731006},
archivePrefix = {arXiv},
       eprint = {1801.08897},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018A&A...612A..47C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Chandra2016InJPh..90..733C,
       author = {{Chandra}, S. and {Sakshi} and {Sharma}, M.~K. and {Kumar}, N.},
        title = "{Methanimine in interstellar medium: line intensities}",
      journal = {Indian Journal of Physics},
         year = "2016",
        month = "Jul",
       volume = {90},
       number = {7},
        pages = {733-739},
          doi = {10.1007/s12648-015-0813-6},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016InJPh..90..733C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Michael1963_10.1021/ja00892a004,
author = {Michael, Joe V. and Noyes, W. Albert.},
title = {The Photochemistry of Methylamine},
journal = {Journal of the American Chemical Society},
volume = {85},
number = {9},
pages = {1228-1233},
year = {1963},
doi = {10.1021/ja00892a004},

URL = { 
        https://doi.org/10.1021/ja00892a004
    
},
eprint = { 
        https://doi.org/10.1021/ja00892a004
    
}

}

@ARTICLE{Acquista1968JChPh..48.1534A,
       author = {{Acquista}, Nicolo and {Schoen}, Louis J. and {Lide}, David R., Jr.},
        title = "{Infrared Spectrum of the Matrix-Isolated OH Radical}",
      journal = {\jcp},
         year = "1968",
        month = "Feb",
       volume = {48},
       number = {4},
        pages = {1534-1536},
          doi = {10.1063/1.1668875},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1968JChPh..48.1534A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Skouteris2015AA...584A..76S,
       author = {{Skouteris}, Dimitrios and {Balucani}, Nadia and {Faginas-Lago}, Noelia and
         {Falcinelli}, Stefano and {Rosi}, Marzio},
        title = "{Dimerization of methanimine and its charged species in the atmosphere of Titan and interstellar/cometary ice analogs}",
      journal = {\aap},
     keywords = {ISM: molecules, planets and satellites: individual: Titan},
         year = "2015",
        month = "Dec",
       volume = {584},
          eid = {A76},
        pages = {A76},
          doi = {10.1051/0004-6361/201526978},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015A&A...584A..76S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Larson2006JChPh.125m3302L,
       author = {{Larson}, Christopher and {Ji}, Yuanyuan and {Samartzis}, Petros and
         {Wodtke}, Alec M. and {Lee}, Shih-Huang and {Lin}, Jim-Min, Jr. and
         {Chaudhuri}, Chanchal and {Ching}, Tao-Tsung},
        title = "{Collision-free photochemistry of methylazide: Observation of unimolecular decomposition of singlet methylnitrene}",
      journal = {\jcp},
     keywords = {82.50.-m, 82.30.Lp, 82.30.Qt, Photochemistry, Decomposition reactions, Isomerization and rearrangement},
         year = "2006",
        month = "Oct",
       volume = {125},
       number = {13},
        pages = {133302-133302},
          doi = {10.1063/1.2215598},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006JChPh.125m3302L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Teslja2004JPCA..108.4433T,
       author = {{Teslja}, Alexey and {Nizamov}, Boris and {Dagdigian}, Paul J.},
        title = "{The Electronic Spectrum of Methyleneimine}",
      journal = {Journal of Physical Chemistry A},
         year = "2004",
        month = "May",
       volume = {108},
       number = {20},
        pages = {4433-4439},
          doi = {10.1021/jp037938+},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2004JPCA..108.4433T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Jacox1975333,
title = "The infrared spectrum of methylenimine",
journal = "Journal of Molecular Spectroscopy",
volume = "56",
number = "3",
pages = "333 - 356",
year = "1975",
issn = "0022-2852",
doi = "https://doi.org/10.1016/0022-2852(75)90122-8",
url = "http://www.sciencedirect.com/science/article/pii/0022285275901228",
author = "Marilyn E. Jacox and Dolphus E. Milligan",
abstract = "Eleven isotopic species of methylenimine have been prepared by the mercury-arc photolysis of methyl azide isolated in argon, nitrogen, and carbon dioxide matrices at 4 and at 14 K. Sufficient concentrations of methylenimine were obtained for identification of all of the vibrational fundamentals except the NH stretching mode. Using a recent ab initio structural calculation for this molecule, it has been possible to derive a set of valence-force potential constants which provide a satisfactory fit to all of the infrared spectroscopic data. The magnitude of the carbon-nitrogen stretching force constant is appropriate for a double bond. The temperature dependence of the thermodynamic properties of methylenimine has also been calculated."
}

@ARTICLE{Bernstein1995ApJ...454..327B,
       author = {{Bernstein}, Max P. and {Sandford}, Scott A. and {Allamand
        ola}, Louis J. and {Chang}, Sherwood and {Scharberg}, Maureen A.},
        title = "{Organic Compounds Produced by Photolysis of Realistic Interstellar and Cometary Ice Analogs Containing Methanol}",
      journal = {\apj},
     keywords = {ISM: DUST, EXTINCTION, INFRARED: ISM: LINES AND BANDS, ISM: MOLECULES, MOLECULAR PROCESSES},
         year = "1995",
        month = "Nov",
       volume = {454},
        pages = {327},
          doi = {10.1086/176485},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1995ApJ...454..327B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Guille2003AA...412..121M,
       author = {{Mu{\~n}oz Caro}, G.~M. and {Schutte}, W.~A.},
        title = "{UV-photoprocessing of interstellar ice analogs: New infrared spectroscopic results}",
      journal = {\aap},
     keywords = {infrared: ISM, ISM: lines and bands, methods: laboratory, ultraviolet: ISM, ISM: dust, extinction},
         year = 2003,
        month = dec,
       volume = {412},
        pages = {121-132},
          doi = {10.1051/0004-6361:20031408},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2003A&A...412..121M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Fox1970Sci...170..984F,
       author = {{Fox}, Sidney W. and {Windsor}, Charles R.},
        title = "{Synthesis of Amino Acids by the Heating of Formaldehyde and Ammonia}",
      journal = {Science},
         year = 1970,
        month = nov,
       volume = {170},
       number = {3961},
        pages = {984-986},
          doi = {10.1126/science.170.3961.984},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1970Sci...170..984F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Meissner1954doi:10.1021/ie50532a035,
author = {Meissner, Fritz and Schwiedessen, Ernst and Othmer, Donald F.},
title = {Continuous Production of Hexamethylenetetramine},
journal = {Industrial \& Engineering Chemistry},
volume = {46},
number = {4},
pages = {724-727},
year = {1954},
doi = {10.1021/ie50532a035},

URL = { 
        https://doi.org/10.1021/ie50532a035
    
},
eprint = { 
        https://doi.org/10.1021/ie50532a035
    
}

}

@ARTICLE{Hamada1984JMoSp.105...70H,
       author = {{Hamada}, Yoshiaki and {Hashiguchi}, Kazuko and {Tsuboi}, Masamichi and
         {Koga}, Yoshinori and {Kondo}, Shigeo},
        title = "{Pyrolysis of amines: Infrared spectrum of methyleneimine}",
      journal = {Journal of Molecular Spectroscopy},
         year = 1984,
        month = may,
       volume = {105},
       number = {1},
        pages = {70-80},
          doi = {10.1016/0022-2852(84)90104-8},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1984JMoSp.105...70H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Gerakines2004Icar..170..202G,
       author = {{Gerakines}, P.~A. and {Moore}, M.~H. and {Hudson}, R.~L.},
        title = "{Ultraviolet photolysis and proton irradiation of astrophysical ice analogs containing hydrogen cyanide}",
      journal = {\icarus},
         year = 2004,
        month = jul,
       volume = {170},
       number = {1},
        pages = {202-213},
          doi = {10.1016/j.icarus.2004.02.005},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2004Icar..170..202G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Purnell1976CP.....12...77P,
       author = {{Purnell}, C.~J. and {Barnes}, A.~J. and {Suzuki}, S. and {Ball}, D.~F. and
         {Orville-Thomas}, W.~J.},
        title = "{Infrared and Raman matrix isolation studies of methylamine}",
      journal = {Chemical Physics},
         year = 1976,
        month = jan,
       volume = {12},
       number = {1},
        pages = {77-87},
          doi = {10.1016/0301-0104(76)80114-0},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1976CP.....12...77P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kaifu1974ApJ...191L.135K,
       author = {{Kaifu}, N. and {Morimoto}, M. and {Nagane}, K. and {Akabane}, K. and
         {Iguchi}, T. and {Takagi}, K.},
        title = "{Detection of Interstellar Methylamine}",
      journal = {\apjl},
         year = 1974,
        month = aug,
       volume = {191},
        pages = {L135-L137},
          doi = {10.1086/181569},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1974ApJ...191L.135K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Fourikis1974ApJ...191L.139F,
       author = {{Fourikis}, N. and {Takagi}, K. and {Morimoto}, M.},
        title = "{Detection of Interstellar Methylamine by its 2\_\{02\}-\&gt;1\_\{10\} A\_\{a\^\{-\}\} State Transition}",
      journal = {\apjl},
         year = 1974,
        month = aug,
       volume = {191},
        pages = {L139},
          doi = {10.1086/181570},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1974ApJ...191L.139F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@Article{Lafosse2006B613479C,
author ="Lafosse, Anne and Bertin, Mathieu and Domaracka, Alicja and Pliszka, Damian and Illenberger, Eugen and Azria, Roger",
title  ="Reactivity induced at 25 K by low-energy electron irradiation of condensed NH3–CH3COOD (1 : 1) mixture",
journal  ="Phys. Chem. Chem. Phys.",
year  ="2006",
volume  ="8",
issue  ="47",
pages  ="5564-5568",
publisher  ="The Royal Society of Chemistry",
doi  ="10.1039/B613479C",
url  ="http://dx.doi.org/10.1039/B613479C",
abstract  ="Chemical reactivity is observed following electron irradiation of a binary mixture of ammonia (NH) and acetic acid (CHCOOD) at 25 K{,} without any subsequent thermal activation{,} as evidenced by vibrational high resolution electron energy loss spectroscopy (HREELS). Analysis of the HREEL spectra and comparison with infrared and Raman data of different molecules are compatible with glycine formation in its zwitterionic form. The onset for electron induced reaction is found to be at about ∼13 eV. The mechanisms may involve NH radicals interaction with CHCOOD molecules. Then glycine formation does not imply any displacement of reactants{,} so that it involves only NH and CHCOOD neighboring molecules."}

@ARTICLE{Holtom2005ApJ...626..940H,
       author = {{Holtom}, Philip D. and {Bennett}, Chris J. and {Osamura}, Yoshihiro and
         {Mason}, Nigel J. and {Kaiser}, Ralf I.},
        title = "{A Combined Experimental and Theoretical Study on the Formation of the Amino Acid Glycine (NH$_{2}$CH$_{2}$COOH) and Its Isomer (CH$_{3}$NHCOOH) in Extraterrestrial Ices}",
      journal = {\apj},
     keywords = {Astrobiology, Astrochemistry, ISM: Cosmic Rays, ISM: General, ISM: Molecules, Molecular Processes},
         year = 2005,
        month = jun,
       volume = {626},
       number = {2},
        pages = {940-952},
          doi = {10.1086/430106},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2005ApJ...626..940H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Hamada1984JMoSp.105...93H,
       author = {{Hamada}, Yoshiaki and {Hashiguchi}, Kazuko and {Tsuboi}, Masamichi and
         {Koga}, Yoshinori and {Kondo}, Shigeo},
        title = "{Pyrolysis of amines: Infrared spectrum of vinylamine}",
      journal = {Journal of Molecular Spectroscopy},
         year = 1984,
        month = may,
       volume = {105},
       number = {1},
        pages = {93-104},
          doi = {10.1016/0022-2852(84)90106-1},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1984JMoSp.105...93H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Dyke1989IJMSI..94..221D,
       author = {{Dyke}, J.~M. and {Lee}, E.~P.~F. and {Zamanpour Niavaran}, M.~H.},
        title = "{A study of the aminomethyl radical CH2NH2 by vacuum UV photoelectron spectroscopy and ab initio molecular orbital calculations}",
      journal = {International Journal of Mass Spectrometry and Ion Processes},
         year = 1989,
        month = nov,
       volume = {94},
       number = {3},
        pages = {221-235},
          doi = {10.1016/0168-1176(89)80044-8},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1989IJMSI..94..221D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Danger2011AA...535A..47D,
       author = {{Danger}, G. and {Borget}, F. and {Chomat}, M. and {Duvernay}, F. and
         {Theul{\'e}}, P. and {Guillemin}, J. -C. and
         {Le Sergeant D'Hendecourt}, L. and {Chiavassa}, T.},
        title = "{Experimental investigation of aminoacetonitrile formation through the Strecker synthesis in astrophysical-like conditions: reactivity of methanimine (CH$_{2}$NH), ammonia (NH$_{3}$), and hydrogen cyanide (HCN)}",
      journal = {A&A},
     keywords = {astrochemistry, ISM: molecules, methods: laboratory},
         year = 2011,
        month = nov,
       volume = {535},
          eid = {A47},
        pages = {A47},
          doi = {10.1051/0004-6361/201117602},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011A&A...535A..47D},
}

@ARTICLE{Danger2011AA...525A..30D,
       author = {{Danger}, G. and {Bossa}, J. -B. and {de Marcellus}, P. and
         {Borget}, F. and {Duvernay}, F. and {Theul{\'e}}, P. and
         {Chiavassa}, T. and {D'Hendecourt}, L.},
        title = "{Experimental investigation of nitrile formation from VUV photochemistry of interstellar ices analogs: acetonitrile and amino acetonitrile}",
      journal = {\aap},
     keywords = {astrochemistry, ISM: molecules, methods: laboratory},
         year = 2011,
        month = jan,
       volume = {525},
          eid = {A30},
        pages = {A30},
          doi = {10.1051/0004-6361/201015736},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011A&A...525A..30D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bogelund2019AA...624A..82B,
       author = {{B{\o}gelund}, Eva G. and {McGuire}, Brett A. and
         {Hogerheijde}, Michiel R. and {van Dishoeck}, Ewine F. and
         {Ligterink}, Niels F.~W.},
        title = "{Methylamine and other simple N-bearing species in the hot cores NGC 6334I MM1-3}",
      journal = {\aap},
     keywords = {astrochemistry, methods: observational, stars: protostars, ISM: individual objects: NGC 6334I, submillimeter: ISM, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2019,
        month = apr,
       volume = {624},
          eid = {A82},
        pages = {A82},
          doi = {10.1051/0004-6361/201833676},
archivePrefix = {arXiv},
       eprint = {1902.07060},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019A&A...624A..82B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Goesmann2015Sci...349b0689G,
       author = {{Goesmann}, Fred and {Rosenbauer}, Helmut and
         {Bredeh{\"o}ft}, Jan Hendrik and {Cabane}, Michel and
         {Ehrenfreund}, Pascale and {Gautier}, Thomas and {Giri}, Chaitanya and
         {Kr{\"u}ger}, Harald and {Le Roy}, L{\'e}na and {MacDermott}, Alexand
        ra J. and {McKenna-Lawlor}, Susan and {Meierhenrich}, Uwe J. and
         {Caro}, Guillermo M. Mu{\~n}oz and {Raulin}, Francois and
         {Roll}, Reinhard and {Steele}, Andrew and {Steininger}, Harald and
         {Sternberg}, Robert and {Szopa}, Cyril and {Thiemann}, Wolfram and
         {Ulamec}, Stephan},
        title = "{Organic compounds on comet 67P/Churyumov-Gerasimenko revealed by COSAC mass spectrometry}",
      journal = {Science},
     keywords = {PLANET SCI},
         year = 2015,
        month = jul,
       volume = {349},
       number = {6247},
        pages = {2.689},
          doi = {10.1126/science.aab0689},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015Sci...349b0689G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kim2011ApJ...729...68K,
       author = {{Kim}, Y.~S. and {Kaiser}, R.~I.},
        title = "{On the Formation of Amines (RNH$_{2}$) and the Cyanide Anion (CN$^{-}$) in Electron-irradiated Ammonia-hydrocarbon Interstellar Model Ices}",
      journal = {\apj},
     keywords = {astrobiology, astrochemistry, cosmic rays, ISM: individual objects: Sagittarius B2, ISM: molecules, methods: laboratory},
         year = 2011,
        month = mar,
       volume = {729},
       number = {1},
          eid = {68},
        pages = {68},
          doi = {10.1088/0004-637X/729/1/68},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011ApJ...729...68K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Forstel2017ApJ...845...83F,
       author = {{F{\"o}rstel}, Marko and {Bergantini}, Alexandre and
         {Maksyutenko}, Pavlo and {G{\'o}bi}, S{\'a}ndor and {Kaiser}, Ralf I.},
        title = "{Formation of Methylamine and Ethylamine in Extraterrestrial Ices and Their Role as Fundamental Building Blocks of Proteinogenic {\ensuremath{\alpha}}-amino Acids}",
      journal = {\apj},
     keywords = {astrochemistry, comets: general, cosmic rays, infrared: ISM, methods: laboratory: molecular, molecular processes},
         year = 2017,
        month = aug,
       volume = {845},
       number = {1},
          eid = {83},
        pages = {83},
          doi = {10.3847/1538-4357/aa7edd},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017ApJ...845...83F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Dickens1997ApJ...479..307D,
       author = {{Dickens}, J.~E. and {Irvine}, W.~M. and {DeVries}, C.~H. and
         {Ohishi}, M.},
        title = "{Hydrogenation of Interstellar Molecules: A Survey for Methylenimine (CH$_{2}$NH)}",
      journal = {\apj},
     keywords = {ISM: Abundances, ISM: Molecules},
         year = 1997,
        month = apr,
       volume = {479},
       number = {1},
        pages = {307-312},
          doi = {10.1086/303884},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1997ApJ...479..307D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Belloche2013AA...559A..47B,
       author = {{Belloche}, A. and {M{\"u}ller}, H.~S.~P. and {Menten}, K.~M. and
         {Schilke}, P. and {Comito}, C.},
        title = "{Complex organic molecules in the interstellar medium: IRAM 30 m line survey of Sagittarius B2(N) and (M)}",
      journal = {\aap},
     keywords = {astrobiology, astrochemistry, line: identification, stars: formation, ISM: individual objects: Sagittarius B2, ISM: molecules, Astrophysics - Astrophysics of Galaxies},
         year = 2013,
        month = nov,
       volume = {559},
          eid = {A47},
        pages = {A47},
          doi = {10.1051/0004-6361/201321096},
archivePrefix = {arXiv},
       eprint = {1308.5062},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013A&A...559A..47B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Altwegg2017MNRAS.469S.130A,
       author = {{Altwegg}, Kathrin and {Balsiger}, H. and {Berthelier}, J.~J. and
         {Bieler}, A. and {Calmonte}, U. and {Fuselier}, S.~A. and
         {Goesmann}, F. and {Gasc}, S. and {Gombosi}, T.~I. and {Le Roy}, L. and
         {de Keyser}, J. and {Morse}, A. and {Rubin}, M. and {Schuhmann}, M. and
         {Taylor}, M.~G.~G.~T. and {Tzou}, C. -Y. and {Wright}, I.},
        title = "{Organics in comet 67P - a first comparative analysis of mass spectra from ROSINA-DFMS, COSAC and Ptolemy}",
      journal = {\mnras},
     keywords = {comets: general, comets: individual: 67P/Churyumov, Gerasimenko},
         year = 2017,
        month = jul,
       volume = {469},
        pages = {S130-S141},
          doi = {10.1093/mnras/stx1415},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017MNRAS.469S.130A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Ehrenfreund2000ARA&A..38..427E,
       author = {{Ehrenfreund}, Pascale and {Charnley}, Steven B.},
        title = "{Organic Molecules in the Interstellar Medium, Comets, and Meteorites: A Voyage from Dark Clouds to the Early Earth}",
      journal = {\araa},
     keywords = {MOLECULAR CLOUDS, SOLAR SYSTEM, CARBON CHEMISTRY, ORIGIN OF LIFE, ASTROBIOLOGY},
         year = 2000,
        month = jan,
       volume = {38},
        pages = {427-483},
          doi = {10.1146/annurev.astro.38.1.427},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2000ARA&A..38..427E},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Pagani2017A&A...604A..32P,
       author = {{Pagani}, L. and {Favre}, C. and {Goldsmith}, P.~F. and {Bergin}, E.~A. and
         {Snell}, R. and {Melnick}, G.},
        title = "{The complexity of Orion: an ALMA view. I. Data and first results}",
      journal = {\aap},
     keywords = {ISM: clouds, ISM: structure, ISM: individual objects: Orion-KL (except planetary nebulae), astrochemistry, molecular processes},
         year = 2017,
        month = jul,
       volume = {604},
          eid = {A32},
        pages = {A32},
          doi = {10.1051/0004-6361/201730466},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017A&A...604A..32P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Ohishi201910.1093/pasj/psz068,
    author = {Ohishi, Masatoshi and Suzuki, Taiki and Hirota, Tomoya and Saito, Masao and Kaifu, Norio},
    title = "{Detection of a new methylamine (CH3NH2) source: Candidate for future glycine surveys}",
    journal = {Publications of the Astronomical Society of Japan},
    volume = {71},
    number = {4},
    year = {2019},
    month = {07},
    abstract = "{Interstellar glycine (NH2CH2COOH), the simplest amino acid, has long been sought in studying a possible relation between the Universe and origin of life. In the last 40 or so years all surveys of glycine have failed; an alternative strategy would be to search for precursor(s) to glycine. Such studies of precursors would be crucial prior to conducting sensitive surveys with ALMA. Laboratory studies have suggested that CH3NH2 is a possible precursor to glycine. Further theoretical study also suggests that the CH2NH2 radical that can be formed from CH3NH2 through photodissociation can be a good precursor to glycine. Thus, we have looked for CH3NH2 towards several hot core sources using the Nobeyama 45 m radio telescope, and succeeded in finding a new CH3NH2 source, G10.47+0.03, with a fractional abundance of 1.5 ± 1.1 × 10−8; at the time of writing, this source is the most abundant source of CH3NH2 ever known. We found that the observed abundance of CH3NH2 agrees fairly well with the theoretical value predicted by R. T. Garrod (2013, ApJ, 765, 60). The detectability of interstellar glycine is discussed.}",
    issn = {0004-6264},
    doi = {10.1093/pasj/psz068},
    url = {https://doi.org/10.1093/pasj/psz068},
    note = {86},
    eprint = {https://academic.oup.com/pasj/article-pdf/71/4/86/29163361/psz068.pdf},
}

@ARTICLE{Sandford2006Sci...314.1720S,
       author = {{Sandford}, Scott A. and {Al{\'e}on}, J{\'e}r{\^o}me and {Alexand
        er}, Conel M.~O. 'D. and {Araki}, Tohru and {Bajt}, Sa{\v{s}}a{\v{a}} and
         {Baratta}, Giuseppe A. and {Borg}, Janet and {Bradley}, John P. and
         {Brownlee}, Donald E. and {Brucato}, John R. and {Burchell}, Mark J. and
         {Busemann}, Henner and {Butterworth}, Anna and {Clemett}, Simon J. and
         {Cody}, George and {Colangeli}, Luigi and {Cooper}, George and
         {D'Hendecourt}, Louis and {Djouadi}, Zahia and {Dworkin}, Jason P. and
         {Ferrini}, Gianluca and {Fleckenstein}, Holger and {Flynn}, George J. and
         {Franchi}, Ian A. and {Fries}, Marc and {Gilles}, Mary K. and
         {Glavin}, Daniel P. and {Gounelle}, Matthieu and {Grossemy}, Faustine and
         {Jacobsen}, Chris and {Keller}, Lindsay P. and {Kilcoyne}, A.~L. David and
         {Leitner}, Jan and {Matrajt}, Graciela and {Meibom}, Anders and
         {Mennella}, Vito and {Mostefaoui}, Smail and {Nittler}, Larry R. and
         {Palumbo}, Maria E. and {Papanastassiou}, Dimitri A. and
         {Robert}, Fran{\c{c}}ois and {Rotundi}, Alessandra and
         {Snead}, Christopher J. and {Spencer}, Maegan K. and
         {Stadermann}, Frank J. and {Steele}, Andrew and {Stephan}, Thomas and
         {Tsou}, Peter and {Tyliszczak}, Tolek and {Westphal}, Andrew J. and
         {Wirick}, Sue and {Wopenka}, Brigitte and {Yabuta}, Hikaru and
         {Zare}, Richard N. and {Zolensky}, Michael E.},
        title = "{Organics Captured from Comet 81P/Wild 2 by the Stardust Spacecraft}",
      journal = {Science},
     keywords = {Planet Sci},
         year = 2006,
        month = dec,
       volume = {314},
       number = {5806},
        pages = {1720},
          doi = {10.1126/science.1135841},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006Sci...314.1720S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{GARDNER1980353,
title = "Methylamine formation in the vacuum ultraviolet photolysis of methane and ammonia mixtures",
journal = "Journal of Photochemistry",
volume = "13",
number = "4",
pages = "353 - 356",
year = "1980",
issn = "0047-2670",
doi = "https://doi.org/10.1016/0047-2670(80)80027-X",
url = "http://www.sciencedirect.com/science/article/pii/004726708080027X",
author = "Edward P. Gardner and James R. McNesby"
}

@ARTICLE{Bossa2009AA...506..601B,
       author = {{Bossa}, J. -B. and {Duvernay}, F. and {Theul{\'e}}, P. and
         {Borget}, F. and {D'Hendecourt}, L. and {Chiavassa}, T.},
        title = "{Methylammonium methylcarbamate thermal formation in interstellar ice analogs: a glycine salt precursor in protostellar environments}",
      journal = {\aap},
     keywords = {astrochemistry, ISM: molecules, methods: laboratory},
         year = 2009,
        month = nov,
       volume = {506},
       number = {2},
        pages = {601-608},
          doi = {10.1051/0004-6361/200912850},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2009A&A...506..601B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Lee2009ApJ...697..428L,
       author = {{Lee}, Chang-Woo and {Kim}, Joon-Ki and {Moon}, Eui-Seong and
         {Minh}, Y.~C. and {Kang}, Heon},
        title = "{Formation of Glycine on Ultraviolet-Irradiated Interstellar Ice-Analog Films and Implications for Interstellar Amino Acids}",
      journal = {\apj},
     keywords = {astrobiology, astrochemistry, ISM: molecules, methods: laboratory, molecular processes, ultraviolet: ISM},
         year = 2009,
        month = may,
       volume = {697},
       number = {1},
        pages = {428-435},
          doi = {10.1088/0004-637X/697/1/428},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2009ApJ...697..428L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Jimenez2014ApJ...788...19J,
       author = {{Jim{\'e}nez-Escobar}, A. and {Giuliano}, B.~M. and
         {Mu{\~n}oz Caro}, G.~M. and {Cernicharo}, J. and {Marcelino}, N.},
        title = "{Investigation of HNCO Isomer Formation in Ice Mantles by UV and Thermal Processing: An Experimental Approach}",
      journal = {\apj},
     keywords = {astrochemistry, infrared: ISM, ISM: molecules, methods: laboratory: solid state, techniques: spectroscopic, ultraviolet: ISM, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Astrophysics of Galaxies, Physics - Chemical Physics},
         year = 2014,
        month = jun,
       volume = {788},
       number = {1},
          eid = {19},
        pages = {19},
          doi = {10.1088/0004-637X/788/1/19},
archivePrefix = {arXiv},
       eprint = {1407.1242},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014ApJ...788...19J},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Broekhuizen2004AA...415..425V,
       author = {{van Broekhuizen}, F.~A. and {Keane}, J.~V. and {Schutte}, W.~A.},
        title = "{A quantitative analysis of OCN$^{-}$ formation in interstellar ice analogs}",
      journal = {\aap},
     keywords = {methods: laboratory, ISM: molecules, ISM: lines and bands, Astrophysics},
         year = 2004,
        month = feb,
       volume = {415},
        pages = {425-436},
          doi = {10.1051/0004-6361:20034161},
archivePrefix = {arXiv},
       eprint = {astro-ph/0311617},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2004A&A...415..425V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{GERAKINES2004202,
title = "Ultraviolet photolysis and proton irradiation of astrophysical ice analogs containing hydrogen cyanide",
journal = "Icarus",
volume = "170",
number = "1",
pages = "202 - 213",
year = "2004",
issn = "0019-1035",
doi = "https://doi.org/10.1016/j.icarus.2004.02.005",
url = "http://www.sciencedirect.com/science/article/pii/S0019103504000685",
author = "P.A. Gerakines and M.H. Moore and R.L. Hudson",
keywords = "Ices, Comets, Radiation chemistry, Photochemistry, Spectroscopy",
abstract = "Hydrogen cyanide (HCN) has been identified in the gas phase of the interstellar medium as well as in the comae of several comets. Terrestrially, HCN is a key component in the synthesis of biologically important molecules such as amino acids. In this paper, we report the results of low-temperature (18 K) ice energetic processing experiments involving pure HCN and mixtures of HCN with H2O and NH3. Ice films, 0.1 to several microns in thickness, were exposed to either ultraviolet photons (110–250 nm) or 0.8-MeV protons to simulate the effects of space environments. Observed products include HCNO (isocyanic acid), NH4+ (ammonium ion), CN− (cyanide ion), OCN− (cyanate ion), HCONH2 (formamide), and species spectrally similar to HCN polymers. Product formation rates and HCN destruction rates were determined where possible. Results are discussed in terms of astrophysical situations in the ISM and the Solar System where HCN would likely play an important role in prebiotic chemistry. These results imply that if HCN is present in icy mixtures representative of the ISM or in comets, it will be quickly converted into other species in energetic environments; pure HCN seems to be polymerized by incident radiation."
}

@ARTICLE{Durig1968JChPh..49.2106D,
       author = {{Durig}, J.~R. and {Bush}, S.~F. and {Baglin}, F.~G.},
        title = "{Infrared and Raman Investigation of Condensed Phases of Methylamine and Its Deuterium Derivatives}",
      journal = {\jcp},
         year = 1968,
        month = sep,
       volume = {49},
       number = {5},
        pages = {2106-2117},
          doi = {10.1063/1.1670372},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1968JChPh..49.2106D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Pettersson1999JPCA..103.9154P,
       author = {{Pettersson}, Mika and {Khriachtchev}, Leonid and {Jolkkonen}, Santtu and
         {R{\"a}s{\"a}nen}, Markku},
        title = "{Photochemistry of HNCO in Solid Xe:  Channels of UV Photolysis and Creation of H2NCO Radicals}",
      journal = {Journal of Physical Chemistry A},
         year = 1999,
        month = nov,
       volume = {103},
       number = {45},
        pages = {9154-9162},
          doi = {10.1021/jp992224d},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1999JPCA..103.9154P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Milligan1961JChPh..35.1491M,
       author = {{Milligan}, Dolphus E.},
        title = "{Infrared Spectroscopic Study of the Photolysis of Methyl Azide and Methyl-d$_{3}$ Azide in Solid Argon and Carbon Dioxide}",
      journal = {\jcp},
         year = 1961,
        month = oct,
       volume = {35},
       number = {4},
        pages = {1491-1497},
          doi = {10.1063/1.1732070},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1961JChPh..35.1491M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Reiser1993JChPh..98.8462R,
       author = {{Reiser}, Georg and {Habenicht}, Wieland and {Mueller-Dethlefs}, Klaus},
        title = "{Zero kinetic energy (ZEKE) photoelectron spectroscopy of ammonia by nonresonant two-photon ionization from the neutral ground state}",
      journal = {\jcp},
     keywords = {Ammonia, Ground State, Kinetic Energy, Multiphoton Absorption, Photoelectron Spectroscopy, Cations, Molecular Rotation, Rydberg Series, Vibrational Spectra, Atomic and Molecular Physics},
         year = 1993,
        month = jun,
       volume = {98},
       number = {11},
        pages = {8462-8468},
          doi = {10.1063/1.464505},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1993JChPh..98.8462R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Clutter1969JChPh..51..153C,
       author = {{Clutter}, Dale R. and {Thompson}, Warren E.},
        title = "{Infrared Spectroscopic Study of Polycrystalline NH$_{4}$CN}",
      journal = {\jcp},
         year = 1969,
        month = jul,
       volume = {51},
       number = {1},
        pages = {153-159},
          doi = {10.1063/1.1671702},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1969JChPh..51..153C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Hudson2008AsBio...8..771H,
       author = {{Hudson}, Reggie L. and {Moore}, Marla H. and {Dworkin}, Jason P. and
         {Martin}, Mildred P. and {Pozun}, Zachary D.},
        title = "{Amino Acids from Ion-Irradiated Nitrile-Containing Ices}",
      journal = {Astrobiology},
     keywords = {Amino acids, Ices, Prebiotic chemistry, Radiation chemistry, Infrared spectra},
         year = 2008,
        month = aug,
       volume = {8},
       number = {4},
        pages = {771-779},
          doi = {10.1089/ast.2007.0131},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008AsBio...8..771H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Herbst2009ARAA..47..427H,
       author = {{Herbst}, Eric and {van Dishoeck}, Ewine F.},
        title = "{Complex Organic Interstellar Molecules}",
      journal = {\araa},
         year = 2009,
        month = sep,
       volume = {47},
       number = {1},
        pages = {427-480},
          doi = {10.1146/annurev-astro-082708-101654},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2009ARA&A..47..427H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Briggs1992OLEB...22..287B,
       author = {{Briggs}, R. and {Ertem}, G. and {Ferris}, J.~P. and {Greenberg}, J.~M. and
         {McCain}, P.~J. and {Mendoza-Gomez}, C.~X. and {Schutte}, W.},
        title = "{Comet Halley as an aggregate of interstellar dust and further evidence for the photochemical formation of organics in the interstellar medium}",
      journal = {Origins of Life and Evolution of the Biosphere},
         year = 1992,
        month = sep,
       volume = {22},
       number = {5},
        pages = {287-307},
          doi = {10.1007/BF01810858},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1992OLEB...22..287B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Guille2004AA...413..209M,
       author = {{Mu{\~n}oz Caro}, G.~M. and {Meierhenrich}, U. and {Schutte}, W.~A. and
         {Thiemann}, W.~H. -P. and {Greenberg}, J.~M.},
        title = "{UV-photoprocessing of interstellar ice analogs: Detection of hexamethylenetetramine-based species}",
      journal = {\aap},
     keywords = {ISM: molecules, methods: laboratory, ultraviolet: ISM, ISM: dust, extinction},
         year = 2004,
        month = jan,
       volume = {413},
        pages = {209-216},
          doi = {10.1051/0004-6361:20031447},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2004A&A...413..209M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Carrascosa2020MNRAS.493..821C,
       author = {{Carrascosa}, H. and {Cruz-D{\'\i}az}, G.~A. and
         {Mu{\~n}oz Caro}, G.~M. and {Dartois}, E. and {Chen}, Y. -J.},
        title = "{Photon-induced desorption of larger species in UV-irradiated methane ice}",
      journal = {\mnras},
     keywords = {astrochemistry, methods: laboratory: molecular, ISM: molecules, ultraviolet: ISM, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Earth and Planetary Astrophysics},
         year = 2020,
        month = mar,
       volume = {493},
       number = {1},
        pages = {821-829},
          doi = {10.1093/mnras/staa334},
archivePrefix = {arXiv},
       eprint = {2002.00173},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020MNRAS.493..821C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Stolkin1977CP.....21..327S,
       author = {{Stolkin}, I. and {Ha}, T. -K. and {G{\"u}nthard}, Hs. H.},
        title = "{N-methylmethyleneimine and ethylideneimine: Gas- and matrix-infrared spectra, AB initio calculations and thermodynamic properties}",
      journal = {Chemical Physics},
         year = 1977,
        month = may,
       volume = {21},
       number = {3},
        pages = {327-347},
          doi = {10.1016/0301-0104(77)85189-6},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1977CP.....21..327S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{mencos2018MNRAS.476.5432M,
       author = {{Mencos}, Alejandro and {Krim}, Lahouari},
        title = "{Formation of doubly and triply bonded unsaturated compounds HCN, HNC, and CH$_{2}$NH via N + CH$_{4}$ low-temperature solid state reaction: from molecular clouds to solar system objects}",
      journal = {\mnras},
     keywords = {Astrochemistry, atomic processes, methods: laboratory: atomic, methods: laboratory: molecular, methods: laboratory: solid state, planets and satellites: atmospheres},
         year = 2018,
        month = jun,
       volume = {476},
       number = {4},
        pages = {5432-5441},
          doi = {10.1093/mnras/sty609},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018MNRAS.476.5432M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Milligan1967JChPh..47..278M,
       author = {{Milligan}, Dolphus E. and {Jacox}, Marilyn E.},
        title = "{Spectroscopic Study of the Vacuum-Ultraviolet Photolysis of Matrix-Isolated HCN and Halogen Cyanides. Infrared Spectra of the Species CN and XNC}",
      journal = {\jcp},
         year = 1967,
        month = jul,
       volume = {47},
       number = {1},
        pages = {278-285},
          doi = {10.1063/1.1711859},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1967JChPh..47..278M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Noble2013MNRAS.428.3262N,
       author = {{Noble}, J.~A. and {Theule}, P. and {Borget}, F. and {Danger}, G. and
         {Chomat}, M. and {Duvernay}, F. and {Mispelaer}, F. and {Chiavassa}, T.},
        title = "{The thermal reactivity of HCN and NH$_{3}$ in interstellar ice analogues}",
      journal = {\mnras},
     keywords = {astrochemistry, molecular data, molecular processes, methods: laboratory, ISM: molecules, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2013,
        month = feb,
       volume = {428},
       number = {4},
        pages = {3262-3273},
          doi = {10.1093/mnras/sts272},
archivePrefix = {arXiv},
       eprint = {1210.7066},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013MNRAS.428.3262N},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bernstein1997ApJ...476..932B,
       author = {{Bernstein}, Max P. and {Sandford}, Scott A. and {Allamandola}, Louis J.},
        title = "{The Infrared Spectra of Nitriles and Related Compounds Frozen in Ar and H$_{2}$O}",
      journal = {\apj},
     keywords = {Infrared: General, Methods: Laboratory, Molecular Data},
         year = 1997,
        month = feb,
       volume = {476},
       number = {2},
        pages = {932-942},
          doi = {10.1086/303651},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1997ApJ...476..932B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Hashiguchi1984JMoSp.105...81H,
       author = {{Hashiguchi}, Kazuko and {Hamada}, Yoshiaki and {Tsuboi}, Masamichi and
         {Koga}, Yoshinori and {Kondo}, Shigeo},
        title = "{Pyrolysis of amines: Infrared spectrum of ethylideneimine}",
      journal = {Journal of Molecular Spectroscopy},
         year = 1984,
        month = may,
       volume = {105},
       number = {1},
        pages = {81-92},
          doi = {10.1016/0022-2852(84)90105-X},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1984JMoSp.105...81H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Durig2006JPCA..110.5674D,
       author = {{Durig}, James R. and {Zheng}, Chao and {Gounev}, Todor K. and
         {Herrebout}, Wouter A. and {van der Veken}, Benjamin J.},
        title = "{Conformational Stability From Temperature-Dependent Fourier Transform Infrared Spectra Of Noble Gas Solutions,r0Structural Parameters, and Barriers To Internal Rotation for Ethylamine{\textdagger}}",
      journal = {Journal of Physical Chemistry A},
         year = 2006,
        month = may,
       volume = {110},
       number = {17},
        pages = {5674-5684},
          doi = {10.1021/jp057305q},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006JPCA..110.5674D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{d'Hendecourt1986AAS...64..453D,
       author = {{D'Hendecourt}, L.~B. and {Allamandola}, L.~J.},
        title = "{Time dependent chemistry in dense molecular clouds. III. Infrared band cross sections of molecules in the solid state at 10K.}",
      journal = {\aaps},
     keywords = {Cosmic Dust, Infrared Spectra, Interstellar Chemistry, Molecular Clouds, Solid State, Time Dependence, Interstellar Matter, Spectral Bands, Astrophysics, Infrared Spectra:Interstellar Molecules, Interstellar Molecules:Infrared Spectra, Molecular Clouds:Chemistry},
         year = 1986,
        month = jun,
       volume = {64},
        pages = {453-467},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1986A&AS...64..453D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Ferraro1980ApSpe..34..525F,
       author = {{Ferraro}, John R. and {Sill}, G. and {Fink}, U.},
        title = "{Infrared Intensity Measurements of Cryodeposited Thin Films of NH$_{3}$, NH$_{4}$HS, H$_{2}$S, and Assignments of Absorption Bands}",
      journal = {Applied Spectroscopy},
         year = 1980,
        month = sep,
       volume = {34},
       number = {5},
        pages = {525-533},
          doi = {10.1366/0003702804731339},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1980ApSpe..34..525F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Sivaraman2013AcSpA.105..238S,
       author = {{Sivaraman}, B. and {Raja Sekhar}, B.~N. and {Nair}, B.~G. and
         {Hatode}, V. and {Mason}, N.~J.},
        title = "{Infrared spectrum of formamide in the solid phase}",
      journal = {Spectrochimica Acta Part A: Molecular Spectroscopy},
         year = 2013,
        month = mar,
       volume = {105},
        pages = {238-244},
          doi = {10.1016/j.saa.2012.12.039},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013AcSpA.105..238S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Bossa2012_ch3nh2_VUV,
author = {Bossa, Jean-Baptiste and Borget, Fabien and Duvernay, F. and Danger, Grégoire and Theulé, Patrice and Chiavassa, Thierry},
year = {2012},
month = {01},
pages = {129-137},
title = {Solid-State Methylamine VUV Irradiation Study Using Carbon Monoxide as an H Radical Scavenger},
volume = {65},
journal = {Australian Journal of Chemistry},
doi = {10.1071/CH11409}
}

@ARTICLE{Schutte1993Icar..104..118S,
       author = {{Schutte}, W.~A. and {Allamandola}, L.~J. and {Sandford}, S.~A.},
        title = "{An Experimental Study of the Organic Molecules Produced in Cometary and Interstellar Ice Analogs by Thermal Formaldehyde Reactions}",
      journal = {\icarus},
     keywords = {Comets, Endothermic Reactions, Formaldehyde, Interstellar Chemistry, Interstellar Matter, Astronomical Spectroscopy, Chemical Composition, Coma, Cryogenic Temperature, Ice, Infrared Spectroscopy, Astrophysics},
         year = 1993,
        month = jul,
       volume = {104},
       number = {1},
        pages = {118-137},
          doi = {10.1006/icar.1993.1087},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1993Icar..104..118S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Ruzi2012_radicals_IR,
author = {Ruzi, Mahmut and Anderson, David},
year = {2012},
month = {11},
pages = {194313},
title = {Photodissociation of N-methylformamide isolated in solid parahydrogen},
volume = {137},
journal = {The Journal of chemical physics},
doi = {10.1063/1.4765372}
}

@ARTICLE{Zhang2017JPCA..121.7176Z,
       author = {{Zhang}, Bingbing and {Kong}, Xiangtao and {Jiang}, Shukang and
         {Zhao}, Zhi and {Yang}, Dong and {Xie}, Hua and {Hao}, Ce and
         {Dai}, Dongxu and {Yang}, Xueming and {Liu}, Zhi-Feng and {Jiang}, Ling},
        title = "{Infrared-Vacuum Ultraviolet Spectroscopic and Theoretical Study of Neutral Methylamine Dimer}",
      journal = {Journal of Physical Chemistry A},
         year = 2017,
        month = sep,
       volume = {121},
       number = {38},
        pages = {7176-7182},
          doi = {10.1021/acs.jpca.7b08096},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017JPCA..121.7176Z},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Jimenez-escobar2011AA...536A..91J,
       author = {{Jim{\'e}nez-Escobar}, A. and {Mu{\~n}oz Caro}, G.~M.},
        title = "{Sulfur depletion in dense clouds and circumstellar regions. I. H$_{2}$S ice abundance and UV-photochemical reactions in the H$_{2}$O-matrix}",
      journal = {\aap},
     keywords = {ISM: molecules, methods: laboratory, ultraviolet: ISM, dust, extinction, infrared: ISM, Astrophysics - Earth and Planetary Astrophysics},
         year = 2011,
        month = dec,
       volume = {536},
          eid = {A91},
        pages = {A91},
          doi = {10.1051/0004-6361/201014821},
archivePrefix = {arXiv},
       eprint = {1112.3240},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011A&A...536A..91J},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Fraser2001MNRAS.327.1165F,
       author = {{Fraser}, Helen J. and {Collings}, Mark P. and
         {McCoustra}, Martin R.~S. and {Williams}, David A.},
        title = "{Thermal desorption of water ice in the interstellar medium}",
      journal = {\mnras},
     keywords = {MOLECULAR DATA, MOLECULAR PROCESSES, METHODS: LABORATORY: ISM: MOLECULES, Astrophysics},
         year = 2001,
        month = nov,
       volume = {327},
       number = {4},
        pages = {1165-1172},
          doi = {10.1046/j.1365-8711.2001.04835.x},
archivePrefix = {arXiv},
       eprint = {astro-ph/0107487},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2001MNRAS.327.1165F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{wexler1967ApSRv...1...29W,
       author = {{Wexler}, Arthur},
        title = "{Integrated Intensities of Absorption Bands in Infrared Spectroscopy}",
      journal = {Applied Spectroscopy Reviews},
         year = 1967,
        month = jan,
       volume = {1},
       number = {1},
        pages = {29-98},
          doi = {10.1080/05704926708547581},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1967ApSRv...1...29W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{schnepp1960JChPh..33...49S,
       author = {{Schnepp}, O. and {Dressler}, K.},
        title = "{Absorption Spectra of Solid Xenon, Krypton, and Argon in the Vacuum Ultraviolet}",
      journal = {\jcp},
         year = 1960,
        month = jul,
       volume = {33},
       number = {1},
        pages = {49-55},
          doi = {10.1063/1.1731133},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1960JChPh..33...49S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@Article{SaladinoC2CS35066A,
author ="Saladino, Raffaele and Botta, Giorgia and Pino, Samanta and Costanzo, Giovanna and Di Mauro, Ernesto",
title  ="Genetics first or metabolism first? The formamide clue",
journal  ="Chem. Soc. Rev.",
year  ="2012",
volume  ="41",
issue  ="16",
pages  ="5526-5565",
publisher  ="The Royal Society of Chemistry",
doi  ="10.1039/C2CS35066A",
url  ="http://dx.doi.org/10.1039/C2CS35066A",
}

@ARTICLE{Hagen1981CP.....56..367H,
       author = {{Hagen}, W. and {Tielens}, A.~G.~G.~M. and {Greenberg}, J.~M.},
        title = "{The infrared spectra of amorphous solid water and ice I $_{c}$ between 10 and 140 K}",
      journal = {Chemical Physics},
         year = 1981,
        month = apr,
       volume = {56},
       number = {3},
        pages = {367-379},
          doi = {10.1016/0301-0104(81)80158-9},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1981CP.....56..367H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Shingledecker2020ApJ...888...52S,
       author = {{Shingledecker}, Christopher N. and {Lamberts}, Thanja and
         {Laas}, Jacob C. and {Vasyunin}, Anton and {Herbst}, Eric and
         {K{\"a}stner}, Johannes and {Caselli}, Paola},
        title = "{Efficient Production of S$_{8}$ in Interstellar Ices: The Effects of Cosmic-Ray-driven Radiation Chemistry and Nondiffusive Bulk Reactions}",
      journal = {\apj},
     keywords = {Cosmic rays, Astrochemistry, Interstellar molecules, Dense interstellar clouds, Interstellar dust processes, 329, 75, 849, 371, 838, Astrophysics - Astrophysics of Galaxies, Physics - Chemical Physics},
         year = 2020,
        month = jan,
       volume = {888},
       number = {1},
          eid = {52},
        pages = {52},
          doi = {10.3847/1538-4357/ab5360},
archivePrefix = {arXiv},
       eprint = {1911.01239},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020ApJ...888...52S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Ruf2019ApJ...885L..40R,
       author = {{Ruf}, Alexander and {Bouquet}, Alexis and {Boduch}, Philippe and
         {Schmitt-Kopplin}, Philippe and {Vinogradoff}, Vassilissa and
         {Duvernay}, Fabrice and {Urso}, Riccardo Giovanni and
         {Brunetto}, Rosario and
         {Le Sergeant d{\textquoteright}Hendecourt}, Louis and
         {Mousis}, Olivier and {Danger}, Gr{\'e}goire},
        title = "{Organosulfur Compounds Formed by Sulfur Ion Bombardment of Astrophysical Ice Analogs: Implications for Moons, Comets, and Kuiper Belt Objects}",
      journal = {\apjl},
     keywords = {Comets, Trans-Neptunian objects, Classical Kuiper Belt objects, Astrochemistry, Astrobiology, Experimental techniques, Laboratory astrophysics, 280, 1705, 250, 75, 74, 2078, 2004},
         year = 2019,
        month = nov,
       volume = {885},
       number = {2},
          eid = {L40},
        pages = {L40},
          doi = {10.3847/2041-8213/ab4e9f},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019ApJ...885L..40R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Hudson2018ApJ...867..138H,
       author = {{Hudson}, Reggie L. and {Gerakines}, Perry A.},
        title = "{Infrared Spectra and Interstellar Sulfur: New Laboratory Results for H$_{2}$S and Four Malodorous Thiol Ices}",
      journal = {\apj},
     keywords = {astrobiology, astrochemistry, infrared: ISM, ISM: molecules, molecular data},
         year = 2018,
        month = nov,
       volume = {867},
       number = {2},
          eid = {138},
        pages = {138},
          doi = {10.3847/1538-4357/aae52a},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018ApJ...867..138H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Mousis2017ApJ...835..134M,
       author = {{Mousis}, O. and {Ozgurel}, O. and {Lunine}, J.~I. and
         {Luspay-Kuti}, A. and {Ronnet}, T. and {Pauzat}, F. and
         {Markovits}, A. and {Ellinger}, Y.},
        title = "{Stability of Sulphur Dimers (S$_{2}$) in Cometary Ices}",
      journal = {\apj},
     keywords = {astrobiology, comets: general, comets: individual: 67P\&Churyumov─Gerasimenko, methods: numerical, solid state: volatile, Astrophysics - Earth and Planetary Astrophysics},
         year = 2017,
        month = feb,
       volume = {835},
       number = {2},
          eid = {134},
        pages = {134},
          doi = {10.3847/1538-4357/aa5279},
archivePrefix = {arXiv},
       eprint = {1612.01579},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017ApJ...835..134M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Woods2015MNRAS.450.1256W,
       author = {{Woods}, Paul M. and {Occhiogrosso}, A. and {Viti}, S. and
         {Ka{\v{n}}uchov{\'a}}, Z. and {Palumbo}, M.~E. and {Price}, S.~D.},
        title = "{A new study of an old sink of sulphur in hot molecular cores: the sulphur residue}",
      journal = {\mnras},
     keywords = {astrochemistry, circumstellar matter, stars: formation, ISM: abundances, ISM: molecules, Astrophysics - Solar and Stellar Astrophysics},
         year = 2015,
        month = jun,
       volume = {450},
       number = {2},
        pages = {1256-1267},
          doi = {10.1093/mnras/stv652},
archivePrefix = {arXiv},
       eprint = {1503.07227},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015MNRAS.450.1256W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Jimenez-escobar2012ApJ...751L..40J,
       author = {{Jim{\'e}nez-Escobar}, A. and {Mu{\~n}oz Caro}, G.~M. and
         {Ciaravella}, A. and {Cecchi-Pestellini}, C. and {Candia}, R. and
         {Micela}, G.},
        title = "{Soft X-Ray Irradiation of H$_{2}$S Ice and the Presence of S$_{2}$ in Comets}",
      journal = {\apjl},
     keywords = {ISM: molecules, methods: laboratory, X-rays: ISM},
         year = 2012,
        month = jun,
       volume = {751},
       number = {2},
          eid = {L40},
        pages = {L40},
          doi = {10.1088/2041-8205/751/2/L40},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012ApJ...751L..40J},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Chen2015ApJ...798...80C,
       author = {{Chen}, Y. -J. and {Juang}, K. -J. and {Nuevo}, M. and
         {Jim{\'e}nez-Escobar}, A. and {Mu{\~n}oz Caro}, G.~M. and
         {Qiu}, J. -M. and {Chu}, C. -C. and {Yih}, T. -S. and {Wu}, C. -Y.~R. and
         {Fung}, H. -S. and {Ip}, W. -H.},
        title = "{Formation of S-bearing Species by VUV/EUV Irradiation of H$_{2}$S-containing Ice Mixtures: Photon Energy and Carbon Source Effects}",
      journal = {\apj},
     keywords = {astrochemistry, methods: laboratory: molecular, molecular processes, ultraviolet: ISM},
         year = 2015,
        month = jan,
       volume = {798},
       number = {2},
          eid = {80},
        pages = {80},
          doi = {10.1088/0004-637X/798/2/80},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015ApJ...798...80C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Oba2020_0c90d3eeb3784052b68673613062d950,
title = "Extraterrestrial hexamethylenetetramine in meteorites—a precursor of prebiotic chemistry in the inner solar system",
author = "Yasuhiro Oba and Yoshinori Takano and Hiroshi Naraoka and Yoshihiro Furukawa and Glavin, {Daniel P.} and Dworkin, {Jason P.} and Shogo Tachibana",
note = "Publisher Copyright: {\textcopyright} 2020, The Author(s). Copyright: Copyright 2020 Elsevier B.V., All rights reserved.",
year = "2020",
month = dec,
doi = "10.1038/s41467-020-20038-x",
language = "English",
volume = "11",
journal = "Nature Communications",
issn = "2041-1723",
publisher = "Nature Publishing Group",
number = "1",
}

@ARTICLE{Vinogradoff2020ECS.....4.1398V,
       author = {{Vinogradoff}, V. and {Remusat}, L. and {McLain}, H.~L. and {Aponte}, J.~C. and {Bernard}, S. and {Danger}, G. and {Dworkin}, J.~P. and {Elsila}, J.~E. and {Jaber}, M.},
        title = "{Impact of Phyllosilicates on Amino Acid Formation under Asteroidal Conditions}",
      journal = {ACS Earth and Space Chemistry},
         year = 2020,
        month = aug,
       volume = {4},
       number = {8},
        pages = {1398-1407},
          doi = {10.1021/acsearthspacechem.0c00137},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020ECS.....4.1398V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Chou2019AIPA....9e5311C,
       author = {{Chou}, Sheng-Lung and {Lo}, Jen-Iu and {Peng}, Yu-Chain and {Lu}, Hsiao-Chi and {Cheng}, Bing-Ming and {Ogilvie}, J.~F.},
        title = "{Emission spectra of atomic and molecular nitrogen from photolysis of ammonia in solid neon}",
      journal = {AIP Advances},
         year = 2019,
        month = may,
       volume = {9},
       number = {5},
          eid = {055311},
        pages = {055311},
          doi = {10.1063/1.5096280},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019AIPA....9e5311C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Materese2020AsBio..20..601M,
       author = {{Materese}, Christopher K. and {Nuevo}, Michel and {Sandford}, Scott A. and {Bera}, Partha P. and {Lee}, Timothy J.},
        title = "{The Production and Potential Detection of Hexamethylenetetramine-Methanol in Space}",
      journal = {Astrobiology},
         year = 2020,
        month = may,
       volume = {20},
       number = {5},
        pages = {601-616},
          doi = {10.1089/ast.2019.2147},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020AsBio..20..601M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Urso2020AA...644A.115U,
       author = {{Urso}, R.~G. and {Vuitton}, V. and {Danger}, G. and {Le Sergeant d'Hendecourt}, L. and {Flandinet}, L. and {Djouadi}, Z. and {Mivumbi}, O. and {Orthous-Daunay}, F.~R. and {Ruf}, A. and {Vinogradoff}, V. and {Wolters}, C. and {Brunetto}, R.},
        title = "{Irradiation dose affects the composition of organic refractory materials in space. Results from laboratory analogues}",
      journal = {\aap},
     keywords = {Kuiper belt: general, astrochemistry, astrobiology, solid state: refractory, methods: laboratory: solid state, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics, Physics - Chemical Physics, Physics - Space Physics},
         year = 2020,
        month = dec,
       volume = {644},
          eid = {A115},
        pages = {A115},
          doi = {10.1051/0004-6361/202039528},
archivePrefix = {arXiv},
       eprint = {2011.08650},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020A&A...644A.115U},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Durig2001_CH3NH2_Kr_Xe,
author = {Durig, James and Zheng, Chao},
year = {2001},
month = {04},
pages = {137-148},
title = {Infrared Spectra of Krypton Solutions of Methylamine},
volume = {12},
journal = {Structural Chemistry - STRUCT CHEM},
doi = {10.1023/A:1016696526207}
}

@ARTICLE{Cottin2001ApJ...561L.139C,
       author = {{Cottin}, H. and {Szopa}, C. and {Moore}, M.~H.},
        title = "{Production of Hexamethylenetetramine in Photolyzed and Irradiated Interstellar Cometary Ice Analogs}",
      journal = {\apjl},
     keywords = {Astrochemistry, Comets: General, ISM: Molecules, Methods: Laboratory, Space Vehicles: Instruments},
         year = 2001,
        month = nov,
       volume = {561},
       number = {1},
        pages = {L139-L142},
          doi = {10.1086/324575},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2001ApJ...561L.139C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Rubin1971ApJ...169L..39R,
       author = {{Rubin}, R.~H. and {Swenson}, G.~W., Jr. and {Benson}, R.~C. and {Tigelaar}, H.~L. and {Flygare}, W.~H.},
        title = "{Microwave Detection of Interstellar Formamide}",
      journal = {\apjl},
         year = 1971,
        month = oct,
       volume = {169},
        pages = {L39},
          doi = {10.1086/180810},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1971ApJ...169L..39R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Oba2019NatCo..10.4413O,
       author = {{Oba}, Yasuhiro and {Takano}, Yoshinori and {Naraoka}, Hiroshi and {Watanabe}, Naoki and {Kouchi}, Akira},
        title = "{Nucleobase synthesis in interstellar ices}",
      journal = {Nature Communications},
         year = 2019,
        month = sep,
       volume = {10},
          eid = {4413},
        pages = {4413},
          doi = {10.1038/s41467-019-12404-1},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019NatCo..10.4413O},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Meierhenrich2005_N-heterocycles,
author = {Meierhenrich, Uwe and Caro, Guillermo and Schutte, Willem and Thiemann, Wolfram and Barbier, Bernard and Brack, Andre},
year = {2005},
month = {08},
pages = {4895-4900},
title = {Precursors of Biological Cofactors from Ultraviolet Irradiation of Circumstellar/Interstellar Ice Analogues},
volume = {11},
journal = {Chem. Eur. J.},
doi = {10.1002/chem.200500074}
}

@misc{gaussian16,
author={M. J. Frisch and G. W. Trucks and H. B. Schlegel and G. E. Scuseria and M. A. Robb and J. R. Cheeseman and G. Scalmani and V. Barone and G. A. Petersson and H. Nakatsuji and X. Li and M. Caricato and A. V. Marenich and J. Bloino and B. G. Janesko and R. Gomperts and B. Mennucci and H. P. Hratchian and J. V. Ortiz and A. F. Izmaylov and J. L. Sonnenberg and D. Williams-Young and F. Ding and F. Lipparini and F. Egidi and J. Goings and B. Peng and A. Petrone and T. Henderson and D. Ranasinghe and V. G. Zakrzewski and J. Gao and N. Rega and G. Zheng and W. Liang and M. Hada and M. Ehara and K. Toyota and R. Fukuda and J. Hasegawa and M. Ishida and T. Nakajima and Y. Honda and O. Kitao and H. Nakai and T. Vreven and K. Throssell and Montgomery, {Jr.}, J. A. and J. E. Peralta and F. Ogliaro and M. J. Bearpark and J. J. Heyd and E. N. Brothers and K. N. Kudin and V. N. Staroverov and T. A. Keith and R. Kobayashi and J. Normand and K. Raghavachari and A. P. Rendell and J. C. Burant and S. S. Iyengar and J. Tomasi and M. Cossi and J. M. Millam and M. Klene and C. Adamo and R. Cammi and J. W. Ochterski and R. L. Martin and K. Morokuma and O. Farkas and J. B. Foresman and D. J. Fox},
title={Gaussian˜16 {R}evision {C}.01},
year={2016},
note={Gaussian Inc. Wallingford CT}
} 

@ARTICLE{sandford1993ApJ...417..815S,
       author = {{Sandford}, Scott A. and {Allamandola}, Louis J.},
        title = "{Condensation and Vaporization Studies of CH 3OH and NH 3 Ices: Major Implications for Astrochemistry}",
      journal = {\apj},
     keywords = {Ammonia, Condensing, Cosmochemistry, Ice, Methyl Alcohol, Sublimation, Vaporizing, Carbon Monoxide, Dust, Infrared Absorption, Infrared Spectra, Molecular Interactions, Surface Energy, Astrophysics, ISM: DUST, EXTINCTION, MOLECULAR PROCESSES},
         year = 1993,
        month = nov,
       volume = {417},
        pages = {815},
          doi = {10.1086/173362},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1993ApJ...417..815S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Sandford2020ChRev.120.4616S,
       author = {{Sandford}, Scott A. and {Nuevo}, Michel and {Bera}, Partha P. and {Lee}, Timothy J.},
        title = "{Prebiotic Astrochemistry and the Formation of Molecules of Astrobiological Interest in Interstellar Clouds and Protostellar Disks}",
      journal = {Chemical Reviews},
         year = 2020,
        month = mar,
       volume = {120},
       number = {11},
        pages = {4616},
          doi = {10.1021/acs.chemrev.9b00560},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020ChRev.120.4616S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bera2019ApJ...884...64B,
       author = {{Bera}, Partha P. and {Sandford}, Scott A. and {Lee}, Timothy J. and {Nuevo}, Michel},
        title = "{The Calculated Infrared Spectra of Functionalized Hexamethylenetetramine (HMT) Molecules}",
      journal = {\apj},
     keywords = {astrobiology, astrochemistry, ISM: molecules, methods: laboratory: molecular, methods: numerical, molecular processes},
         year = 2019,
        month = oct,
       volume = {884},
       number = {1},
          eid = {64},
        pages = {64},
          doi = {10.3847/1538-4357/ab3c4f},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019ApJ...884...64B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Layer1963_chemistry_imines,
author = {Layer, Robert W.},
title = {The Chemistry of Imines.},
journal = {Chemical Reviews},
volume = {63},
number = {5},
pages = {489-510},
year = {1963},
doi = {10.1021/cr60225a003},

URL = { 
        https://doi.org/10.1021/cr60225a003
    
},
eprint = { 
        https://doi.org/10.1021/cr60225a003
    
}

}

@article{Vazart2016_formamide_from_CH2NH_OH,
author = {Vazart, Fanny and Calderini, Danilo and Puzzarini, Cristina and Skouteris, Dimitrios and Barone, Vincenzo},
year = {2016},
month = {09},
pages = {},
title = {State-of-the-Art Thermochemical and Kinetic Computations for Astrochemical Complex Organic Molecules: Formamide Formation in Cold Interstellar Clouds as a Case Study},
volume = {12},
journal = {Journal of chemical theory and computation},
doi = {10.1021/acs.jctc.6b00379}
}

@ARTICLE{bossa2009ApJ...707.1524B,
       author = {{Bossa}, J.~B. and {Theule}, P. and {Duvernay}, F. and {Chiavassa}, T.},
        title = "{NH$_{2}$CH$_{2}$OH Thermal Formation in Interstellar Ices Contribution to the 5-8 {\ensuremath{\mu}}m Region Toward Embedded Protostars}",
      journal = {\apj},
     keywords = {astrochemistry, ISM: molecules, molecular data, molecular processes},
         year = 2009,
        month = dec,
       volume = {707},
       number = {2},
        pages = {1524-1532},
          doi = {10.1088/0004-637X/707/2/1524},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2009ApJ...707.1524B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{MD2020ApJ...894...98M,
       author = {{Mart{\'\i}n-Dom{\'e}nech}, Rafael and {{\"O}berg}, Karin I. and {Rajappan}, Mahesh},
        title = "{Formation of NH$_{2}$CHO and CH$_{3}$CHO upon UV Photoprocessing of Interstellar Ice Analogs}",
      journal = {\apj},
     keywords = {Interstellar molecules, Ice formation, Laboratory astrophysics, 849, 2092, 2004, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Astrophysics of Galaxies, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2020,
        month = may,
       volume = {894},
       number = {2},
          eid = {98},
        pages = {98},
          doi = {10.3847/1538-4357/ab84e8},
archivePrefix = {arXiv},
       eprint = {2004.01151},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020ApJ...894...98M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Martin_domenech2014_TPD_hielos,
	author = {{Martín-Doménech, R.} and {Muñoz Caro, G. M.} and {Bueno, J.} and {Goesmann, F.}},
	title = {Thermal desorption of circumstellar and cometary ice analogs},
	DOI= "10.1051/0004-6361/201322824",
	url= "https://doi.org/10.1051/0004-6361/201322824",
	journal = {A&A},
	year = 2014,
	volume = 564,
	pages = "A8",
	month = "",
}


@article{Pouillot_1996_sublimacion_alcanos,
author = {Pouillot, Frederic L. L. and Chandler, Karen and Eckert, Charles A.},
title = {Sublimation Pressures of n-Alkanes from C20H42 to C35H72 in the Temperature Range 308−348 K},
journal = {Industrial \& Engineering Chemistry Research},
volume = {35},
number = {7},
pages = {2408-2413},
year = {1996},
doi = {10.1021/ie950590n},

URL = { 
    
        https://doi.org/10.1021/ie950590n
    
    

},
eprint = { 
    
        https://doi.org/10.1021/ie950590n
    
    

}

}

@article{cazaux2022_H2S_chains,
  title={Photoprocessing of H2S on dust grains-Building S chains in translucent clouds and comets},
  author={Cazaux, S and Carrascosa, H and Caro, GM Mu{\~n}oz and Caselli, P and Fuente, A and Navarro-Almaida, D and Rivi{\'e}re-Marichalar, P},
  journal={Astronomy \& Astrophysics},
  volume={657},
  pages={A100},
  year={2022},
  publisher={EDP Sciences}
}

@ARTICLE{Jenkins2009_ApJ...700.1299J,
       author = {{Jenkins}, Edward B.},
        title = "{A Unified Representation of Gas-Phase Element Depletions in the Interstellar Medium}",
      journal = {\apj},
     keywords = {ISM: abundances, ISM: atoms, ultraviolet: ISM, Astrophysics - Galaxy Astrophysics},
         year = 2009,
        month = aug,
       volume = {700},
       number = {2},
        pages = {1299-1348},
          doi = {10.1088/0004-637X/700/2/1299},
archivePrefix = {arXiv},
       eprint = {0905.3173},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2009ApJ...700.1299J},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Penzias1971_ApJ...168L..53P,
       author = {{Penzias}, A.~A. and {Solomon}, P.~M. and {Wilson}, R.~W. and {Jefferts}, K.~B.},
        title = "{Interstellar Carbon Monosulfide}",
      journal = {\apjl},
         year = 1971,
        month = sep,
       volume = {168},
        pages = {L53},
          doi = {10.1086/180784},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1971ApJ...168L..53P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{oppenheimer1974_chemistry,
  title={The chemistry of sulfur in interstellar clouds},
  author={Oppenheimer, M and Dalgarno, A},
  journal={The Astrophysical Journal},
  volume={187},
  pages={231--236},
  year={1974}
}

@article{bulut2021_gas_phase_abundances,
  title={Gas phase Elemental abundances in Molecular cloudS (GEMS)-III. Unlocking the CS chemistry: the CS+ O reaction},
  author={Bulut, N and Roncero, O and Aguado, A and Loison, J-C and Navarro-Almaida, D and Wakelam, V and Fuente, A and Roueff, Evelyne and Le Gal, R and Caselli, P and others},
  journal={Astronomy \& Astrophysics},
  volume={646},
  pages={A5},
  year={2021},
  publisher={EDP sciences}
}

@ARTICLE{Calmonet2016_detection_S3_S4_Rosetta,
       author = {{Calmonte}, U. and {Altwegg}, K. and {Balsiger}, H. and {Berthelier}, J.~J. and {Bieler}, A. and {Cessateur}, G. and {Dhooghe}, F. and {van Dishoeck}, E.~F. and {Fiethe}, B. and {Fuselier}, S.~A. and {Gasc}, S. and {Gombosi}, T.~I. and {H{\"a}ssig}, M. and {Le Roy}, L. and {Rubin}, M. and {S{\'e}mon}, T. and {Tzou}, C. -Y. and {Wampfler}, S.~F.},
        title = "{Sulphur-bearing species in the coma of comet 67P/Churyumov-Gerasimenko}",
      journal = {\mnras},
     keywords = {space vehicles, space vehicles: instruments, comets: general, comets: individual: 67P/Churyumov-Gerasimenko},
         year = 2016,
        month = nov,
       volume = {462},
        pages = {S253-S273},
          doi = {10.1093/mnras/stw2601},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016MNRAS.462S.253C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Mahjoub2023_sulfur_species_rosetta,
author = {Mahjoub, Ahmed and Altwegg, Kathrin and Poston, M. and Rubin, Martin and Hodyss, Robert and Choukroun, Mathieu and Ehlmann, Bethany and Hänni, Nora and Brown, Michael and Blacksberg, Jordana and Eiler, John and Hand, Kevin},
year = {2023},
month = {06},
pages = {eadh0394},
title = {Complex organosulfur molecules on comet 67P: Evidence from the ROSINA measurements and insights from laboratory simulations},
volume = {9},
journal = {Science advances},
doi = {10.1126/sciadv.adh0394}
}

@article{mastrapa2009_H2O,
  title={Optical constants of amorphous and crystalline H2O-ice: 2.5--22 $\mu$m (4000--455 cm- 1) optical constants of H2O-ice},
  author={Mastrapa, RM and Sandford, SA and Roush, TL and Cruikshank, DP and Dalle Ore, CM},
  journal={The Astrophysical Journal},
  volume={701},
  number={2},
  pages={1347},
  year={2009},
  publisher={IOP Publishing}
}

@article{Smith1997_volcano_desorption_water,
  title={The Molecular Volcano: Abrupt CC l 4 Desorption Driven by the Crystallization of Amorphous Solid Water},
  author={Smith, R Scott and Huang, Chen and Wong, EKLl and Kay, Bruce D},
  journal={Physical review letters},
  volume={79},
  number={5},
  pages={909},
  year={1997},
  publisher={APS}
}

@article{duley1980_formation_H2S_ISM,
  title={Interstellar chemistry of sulphur},
  author={Duley, WW and Millar, TJ and Williams, DA},
  journal={Monthly Notices of the Royal Astronomical Society, vol. 192, Sept. 1980, p. 945-957. Research supported by the Science Research Council and Natural Sciences and Engineering Research Council of Canada.},
  volume={192},
  pages={945--957},
  year={1980}
}


@Article{Kharma2019_review_polysulfides,
AUTHOR = {Kharma, Ammar and Grman, Marian and Misak, Anton and Domínguez-Álvarez, Enrique and Nasim, Muhammad Jawad and Ondrias, Karol and Chovanec, Miroslav and Jacob, Claus},
TITLE = {Inorganic Polysulfides and Related Reactive Sulfur–Selenium Species from the Perspective of Chemistry},
JOURNAL = {Molecules},
VOLUME = {24},
YEAR = {2019},
NUMBER = {7},
ARTICLE-NUMBER = {1359},
URL = {https://www.mdpi.com/1420-3049/24/7/1359},
PubMedID = {30959902},
ISSN = {1420-3049},
ABSTRACT = {Polysulfides (H2Sx) represent a class of reactive sulfur species (RSS) which includes molecules such as H2S2, H2S3, H2S4, and H2S5, and whose presence and impact in biological systems, when compared to other sulfur compounds, has only recently attracted the wider attention of researchers. Studies in this field have revealed a facet-rich chemistry and biological activity associated with such chemically simple, still unusual inorganic molecules. Despite their chemical simplicity, these inorganic species, as reductants and oxidants, metal binders, surfactant-like “cork screws” for membranes, components of perthiol signalling and reservoirs for inorganic hydrogen sulfide (H2S), are at the centre of complicated formation and transformation pathways which affect numerous cellular processes. Starting from their chemistry, the hidden presence and various roles of polysulfides in biology may become more apparent, despite their lack of clear analytical fingerprints and often murky biochemical footprints. Indeed, the biological chemistry of H2Sx follows many unexplored paths and today, the relationship between H2S and its oxidized H2Sx species needs to be clarified as a matter of “unmistaken identity”. Simultaneously, emerging species, such as HSSeSH and SenS8−n, also need to be considered in earnest.},
DOI = {10.3390/molecules24071359}
}

@ARTICLE{Tesis_guillermo,
       author = {{Mu{\~n}oz Caro}, G.~M.},
        title = "{Ph.D. Thesis}",
      journal = {Ph.D. Thesis},
     keywords = {},
         year = 2002,
        month = {},
       volume = {},
          eid = {},
        pages = {},
          doi = {},
 primaryClass = {},
       adsurl = {},
      adsnote = {}
}

@article{Cristobal2022_CO_density,
    author = {Gonz\'alez D\'iaz, C. and Carrascosa, H. and Mu\~noz Caro, G. M. and Satorre, M. \'A. and Chen, Y.-J.},
    title = "{Density and infrared band strength of interstellar carbon monoxide (CO) ice analogues}",
    journal = {MNRAS},
    volume = {517},
    number = {4},
    pages = {5744-5755},
    year = {2022},
    month = {10},
    abstract = "{The motivation to study experimentally CO ice under mimicked interstellar conditions is supported by the large CO gas abundances and ubiquitous presence of CO in icy grain mantles. Upon irradiation in its pure ice form, this highly stable species presents a limited ion and photon-induced chemistry, and an efficient non-thermal desorption. Using infrared spectroscopy, single laser interference, and quadrupole mass spectrometry during CO ice deposition, the CO ice density was estimated as a function of deposition temperature. Only minor variations in the density were found. The proposed methodology can be used to obtain the density of other ice components at various deposition temperatures provided that this value of the density is known for one of these temperatures, which is typically the temperature corresponding to the crystalline form. The apparent tendency of the CO ice density to decrease at deposition temperatures below 14 K is in line with recently published colorimetric measurements. This work allowed us to revisit the value of the infrared band strength needed for calculation of the CO ice column density in infrared observations, 8.7 × 10−18 cm molecule−1 at 20 K deposition temperature.}",
    issn = {0035-8711},
    doi = {10.1093/mnras/stac3122},
    url = {https://doi.org/10.1093/mnras/stac3122},
    eprint = {https://academic.oup.com/mnras/article-pdf/517/4/5744/48716297/stac3122.pdf},
}

@ARTICLE{Yarnall2022_IR_band_strengths,
       author = {{Yarnall}, Yukiko Y. and {Hudson}, Reggie L.},
        title = "{A New Method for Measuring Infrared Band Strengths in H$_{2}$O Ices: First Results for OCS, H$_{2}$S, and SO$_{2}$}",
      journal = {\apjl},
     keywords = {Interstellar molecules, Astrochemistry, Laboratory astrophysics, Chemical abundances, 849, 75, 2004, 224},
         year = 2022,
        month = may,
       volume = {931},
       number = {1},
          eid = {L4},
        pages = {L4},
          doi = {10.3847/2041-8213/ac6b32},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022ApJ...931L...4Y},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Caselli1994_ApJ...421..206C,
       author = {{Caselli}, P. and {Hasegawa}, T.~I. and {Herbst}, Eric},
        title = "{The Production of Condensed Phase CO in Quiescent Molecular Clouds}",
      journal = {\apj},
     keywords = {Carbon Monoxide, Interplanetary Dust, Methyl Alcohol, Molecular Clouds, Abundance, Astronomical Models, Interstellar Chemistry, Astrophysics, ISM: DUST, EXTINCTION, ISM: CLOUDS, ISM: MOLECULES, MOLECULAR PROCESSES},
         year = 1994,
        month = jan,
       volume = {421},
        pages = {206},
          doi = {10.1086/173637},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1994ApJ...421..206C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Ruffle1999_sulfur_depletion,
       author = {{Ruffle}, D.~P. and {Hartquist}, T.~W. and {Caselli}, P. and {Williams}, D.~A.},
        title = "{The sulphur depletion problem}",
      journal = {\mnras},
         year = 1999,
        month = jul,
       volume = {306},
       number = {3},
        pages = {691-695},
          doi = {10.1046/j.1365-8711.1999.02562.x},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1999MNRAS.306..691R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Laas2019_sulfur_depletion_model,
       author = {{Laas}, Jacob C. and {Caselli}, Paola},
        title = "{Modeling sulfur depletion in interstellar clouds}",
      journal = {\aap},
     keywords = {astrochemistry, molecular processes, ISM: molecules, Astrophysics - Astrophysics of Galaxies},
         year = 2019,
        month = apr,
       volume = {624},
          eid = {A108},
        pages = {A108},
          doi = {10.1051/0004-6361/201834446},
archivePrefix = {arXiv},
       eprint = {1903.01232},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019A&A...624A.108L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Altwegg_2022_sulfur_in_comets,
       author = {{Altwegg}, K. and {Combi}, M. and {Fuselier}, S.~A. and {H{\"a}nni}, N. and {De Keyser}, J. and {Mahjoub}, A. and {M{\"u}ller}, D.~R. and {Pestoni}, B. and {Rubin}, M. and {Wampfler}, S.~F.},
        title = "{Abundant ammonium hydrosulphide embedded in cometary dust grains}",
      journal = {\mnras},
     keywords = {astrochemistry, comets: general, comets: individual: 67P/Churyumov-Gerasimenko, Astrophysics - Earth and Planetary Astrophysics},
         year = 2022,
        month = nov,
       volume = {516},
       number = {3},
        pages = {3900-3910},
          doi = {10.1093/mnras/stac2440},
archivePrefix = {arXiv},
       eprint = {2208.11396},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022MNRAS.516.3900A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Altwegg2019_review_rosetta_ARAA..57..113A,
       author = {{Altwegg}, Kathrin and {Balsiger}, Hans and {Fuselier}, Stephen A.},
        title = "{Cometary Chemistry and the Origin of Icy Solar System Bodies: The View After Rosetta}",
      journal = {\araa},
     keywords = {Astrophysics - Earth and Planetary Astrophysics},
         year = 2019,
        month = aug,
       volume = {57},
        pages = {113-155},
          doi = {10.1146/annurev-astro-091918-104409},
archivePrefix = {arXiv},
       eprint = {1908.04046},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019ARA&A..57..113A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Ferreira_2011_sublimation_sulfur,
author = {Ferreira, A.G.M. and Lobo, L.Q.},
year = {2011},
month = {02},
pages = {95–104},
title = {The low-pressure phase diagram of sulfur},
volume = {43},
journal = {The Journal of Chemical Thermodynamics},
doi = {10.1016/j.jct.2010.07.007}
}

@article{bradley1951_sublimation_rhombic_sulphur,
  title={Rates of evaporation IV. The rate of evaporation and vapour pressure of rhombic sulphur},
  author={Bradley, R-S\_},
  journal={Proceedings of the Royal Society of London. Series A. Mathematical and Physical Sciences},
  volume={205},
  number={1083},
  pages={553--563},
  year={1951},
  publisher={The Royal Society London}
}

@article{briske1960_sulfur_sublimation,
  title={The vapour pressures and latent heats of sublimation of \alpha-, \beta- and \gamma- sulphur},
  author={{Briske}, C. and {Hartshorne}, N. H. and {Stranks}, D. R.},
  journal={J. Chem. Soc.},
  volume={},
  number={},
  pages={1200--1209},
  year={1960},
  publisher={Royal Society of Chemistry}
}

@ARTICLE{Collings_2004_laboratory-to-astrophysical-context,
       author = {{Collings}, Mark P. and {Anderson}, Mark A. and {Chen}, Rui and {Dever}, John W. and {Viti}, Serena and {Williams}, David A. and {McCoustra}, Martin R.~S.},
        title = "{A laboratory survey of the thermal desorption of astrophysically relevant molecules}",
      journal = {\mnras},
     keywords = {astrochemistry, molecular processes, methods: laboratory, stars: formation, ISM: molecules},
         year = 2004,
        month = nov,
       volume = {354},
       number = {4},
        pages = {1133-1140},
          doi = {10.1111/j.1365-2966.2004.08272.x},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2004MNRAS.354.1133C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{cazaux_2015_AA...573A..16C,
       author = {{Cazaux}, S. and {Bossa}, J. -B. and {Linnartz}, H. and {Tielens}, A.~G.~G.~M.},
        title = "{Pore evolution in interstellar ice analogues. Simulating the effects of temperature increase}",
      journal = {\aap},
     keywords = {astrochemistry, ISM: abundances, ISM: molecules, stars: formation, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics},
         year = 2015,
        month = jan,
       volume = {573},
          eid = {A16},
        pages = {A16},
          doi = {10.1051/0004-6361/201424466},
archivePrefix = {arXiv},
       eprint = {1410.6343},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015A&A...573A..16C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
